Vertex Block Descent

We introduce vertex block descent, a block coordinate descent solution for the variational form of implicit Euler through vertex-level Gauss-Seidel iterations. It operates with local vertex position updates that achieve reductions in global variational energy with maximized parallelism. This forms a physics solver that can achieve numerical convergence with unconditional stability and exceptional computation performance. It can also fit in a given computation budget by simply limiting the iteration count while maintaining its stability and superior convergence rate. We present and evaluate our method in the context of elastic body dynamics, providing details of all essential components and showing that it outperforms alternative techniques. In addition, we discuss and show examples of how our method can be used for other simulation systems, including particle-based simulations and rigid bodies.

==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/01_Introduction.tex <==
\section{Introduction}

Physics-based simulation is the cornerstone of most graphics applications and the demands from simulation systems to deliver improved stability, accelerated computational performance, and enhanced visual realism are ever-growing. Particularly in real-time graphics applications, the stability and performance requirements are so strict that realism can sometimes be begrudgingly considered of secondary importance.

Notwithstanding the substantial amount of research and groundbreaking discoveries made on physics solvers over the past decades, existing methods still leave some things to be desired. They either deliver high-quality results, but fail to meet the computational demands of many applications or fit in a given computation time by sacrificing quality. Stability, on the other hand, is always a challenge, particularly with strict computation budgets.

In this paper, we introduce \emph{vertex block descent (VBD)}, a physics solver that offers unconditional stability, superior computational performance than prior methods, and the ability to achieve numerical convergence \add{to an implicit Euler integration}. 
%given a sufficient computation budget.
%This forms a general method that can be applied to a variety of simulation problems. Nonetheless, 
Though our method is a general solution that can be used for a variety of simulation problems, 
we present and evaluate it in the context of elastic body dynamics. Then, we briefly discuss how our method can be applied to some other simulation systems, including particle-based simulations and rigid bodies.

Our VBD method is based on block coordinate descent that performs vertex-based Gauss-Seidel iterations to solve the variational form of implicit Euler.
%
For elastic body dynamics, each iteration runs a loop over the mesh vertices, adjusting the position of a single vertex at a time, temporarily fixing all others. 
%\yin{Since vertex forms the most basic unit of degrees of freedom (DOFs), VBD 
This offers maximized parallelism when coupled with vertex-based mesh coloring, which can achieve an order of magnitude fewer colors (i.e. serialized workloads) as compared to element-based parallelization.
%This provides improved parallelism with vertex-based mesh coloring that results in significantly fewer colors as compared to element-based coloring used by prior methods \cem{cite some}.
Our local position-based updates can ensure that the variational energy is always reduced. 
%Therefore, our method maintains its stability even in challenging cases involving high potential energy, large residuals, and/or only a single iteration per time step.
Therefore, our method maintains its stability even with a single iteration per time step and large time steps, operating with unconverged solutions containing a large amount of residual. With more iterations, it converges faster than its alternatives. Thus, it can more easily fit in a given computation budget, while maintaining stability with improved convergence.

We present all essential components of using VBD for elastic body dynamics, including formulations for damping, constraints, collisions, and friction. We also introduce a simple initialization scheme to warm-start the optimization and improve convergence. In addition, we discuss momentum-based acceleration techniques and parallelization in the presence of dynamic collisions.
%
Our evaluation includes large simulations (\autoref{fig:teaser}) and stress tests (e.g. \autoref{fig:ExtremeTwist} and \ref{fig:ExtremeInitialization}) that demonstrate VBD's performance, scalability, and stability.


%We evaluate our method with various challenging simulation scenarios involving elastic body dynamics and compare its performance to the state-of-the-art methods and the fastest existing simulation systems. Our results show that VBD consistently provides improved convergence and faster performance \cem{mentioning specific numbers here would be nice} than all of them. In addition, we show that VBD maintains its stability even in extreme tests and successfully handles challenging cases, such as extreme mass differences and infinitely stiff materials. Some example results of our method are shown in \autoref{fig:teaser}.

%\cem{It'd be good to highlight the position-based computation aspect here.}


\begin{figure}
\newcommand{\img}[1]{\includegraphics[width=0.5\linewidth,trim=100 230 150 150, clip]{Figures/BeamRotation/#1-cc}}
\centering
%\img{a}\hfill
\img{b}\hfill\img{c}
\caption{Twisting two beams together, totaling 97 thousand vertices and 266 thousand tetrahedra, demonstrating complex frictional contact and buckling.}
\label{fig:ExtremeTwist}
\end{figure}




==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/02_RelatedWorks.tex <==
\section{Related Work}

There is a large body of work on physics-based simulation in computer graphics. Here we only discuss the recent and the most relevant work to our method.



Implicit time integrators are widely accepted as the primary methods for simulating elastic bodies in computer graphics due to their exceptional stability, especially when addressing stiff problems.
Among these options, backward Euler \cite{baraff_large_1998, hirota_implicit_2001, volino_comparing_2001, martin2011example} is the most commonly utilized method, though other approaches like implicit Newmark \cite{kane2000variational, bridson2002robust, bridson2005simulation}, BDF2 \cite{choi_stable_2005, hauth_high_2001}, and implicit-explicit \cite{hansmann_implicit-explicit_2000, stern_implicit-explicit_2009} have also been explored.
%
Backward Euler is often approximated as a single Newton step, solving a linear system of equations \cite{baraff_large_1998}. Line search can be applied to improve robustness \cite{hirota_implicit_2001}.
%The solution of Backward Euler can be addressed by linearizing the force formulation and solving a global (but usually sparse) linear system \cite{baraff_large_1998}. The line search approach can also be applied to the direction given by Newton's method to improve robustness \cite{hirota_implicit_2001}.
Preconditioning \cite{ascher2003modified} or positive-definite projection \cite{teran2005robust} can be used to improve convergence.
%However, addressing such a global linear system is challenging, given its computational expense and vulnerability to inadequate numerical precision, ill-condition, and non-positive-definiteness. To tackle these issues, techniques such as preconditioning \cite{ascher2003modified} or positive-definite projection \cite{teran2005robust} are incorporated to ensure convergence.
To circumvent a full linear solve for every Newton step, Cholesky factorization \cite{hecht_updated_2012} emerges as a viable strategy. 
Techniques like multi-resolution \cite{grinspun2002charms, capell_multiresolution_2002} or multigrid \cite{bolz2003sparse, tamstorf_smoothed_2015, xian_scalable_2019, wang_hierarchical_2020, zhu_efficient_2010} solvers 
%offer alternative methods. These methods involve projecting 
project
finer details onto a coarser grid with fewer degrees of freedom, effectively reducing the computational cost of the linear system solver.
Our solution linearizes the forces locally, avoiding the global linear system, and it converges to the same result as backward Euler with multiple Newton steps.

% Or quasi-Newton method using approximated Hessian: 
Additionally, stiffness warping \cite{muller2002stable} repurposes the stiffness matrix from the rest shape to handle significant rotational deformations. Using a quasi-Newton method \cite{liu_quasi-newton_2017} with an approximate Hessian can be far more cost-effective for computing its inverse with prefactoring than the actual Hessian. Example-based dynamics has also been explored \cite{chao_simple_2010, muller2005meshless, martin2011example}, where the deformation energy is defined based on the nearest point in the example space.
Projective Dynamics \cite{bouaziz2023projective} represents deformation energy via a series of constraints that can be solved independently, then synchronized either through a prefactorized global step to accelerate convergence.
% \cite{fratarcangeli_scalable_2015}, a more general coloring scheme for sparse linear system \cite{fratarcangeli_vivace_2016}, a clustered coloring scheme: \cite{ton-that_parallel_2023}.

The relation between dynamics, energy, and minimization has been leveraged in variational integrators \cite{kane2000variational, kane_symplectic-energy-momentum_1999, simo_exact_1992,lew_variational_2004, 10.2312:SCA:SCA06:043-051}.  Reformulating backward Euler to an optimization problem combined with optimization techniques to allows the usage of large steps \cite{martin2011example, gast_optimization_2015}. Domain-decomposed optimization for solving the nonlinear problems of implicit numerical time integration can accelerate convergence \citet{li_decomposed_2019}. Yet, the optimization formulation has its drawbacks, notably the varying problem formulation and initial positions in each step. Consequently, achieving consistent convergence within a fixed time budget becomes challenging. Real-time simulators compromise by accepting partially converged results, which visually resemble the final solution. Unfortunately, this compromise can lead to significant visual artifacts mainly due to retained residuals from earlier steps, which can accumulate across frames and can jeopardize the solver's stability.
%, potentially resulting in catastrophic simulation failure 
% \autoref{fig:StabilityUnderResidual}. 
Our method, as illustrated in \autoref{fig:ExtremeStretch2}, demonstrates exceptional stability even when retaining a substantial amount of residual with a limited number of iterations.
% However, our method exhibits exceptional stability even while retaining a substantial amount of residual when using a limited number of iterations, see \autoref{fig:ExtremeStretch2}.





\begin{figure}%\vspace{-1em}
\centering
%\includegraphics[width=\columnwidth]{Figures/10_2SquishyballColliding.pdf}
\newcommand{\fig}[2][700 100 640 400]{\includegraphics[width=0.248\linewidth,trim=#1, clip]{Figures/RandomizeAndFlattening/#2-cc}}
\fig{a}\hfill%
\fig{b}\hfill%
\fig{c}\hfill%
\fig[700 300 640 200]{d}
\newcommand{\figT}[1]{\fig[400 200 400 80]{#1}}
\figT{e}\hfill%
\figT{f}\hfill%
\figT{g}\hfill%
\figT{h}
\caption{Stress tests that begin simulations under extreme deformations: \sref{top}~a perfectly flattened armadillo model with 15 thousand vertices and 50 thousand tetrahedra, and \sref{bottom}~a Utah teapot model with 2 thousand vertices and 8.5 thousand tetrahedra, deformed by randomly placing its vertices onto the surface of a sphere. Both models quickly recover to their original shape shortly after the simulation starts. Both simulations use accelerated iterations with $\rho=0.95$.} %(a)-(d) The collision process.
\label{fig:ExtremeInitialization}
%\vspace{1em}
\end{figure}






Position-based dynamics methods (PBD \cite{muller2007position} and XPBD \cite{macklin_xpbd_2016}) convert forces into (soft) constraints and directly update the positions with Gauss-Seidel iterations operating on one constraint at a time. These position-based updates result in exceptional stability, which is often exploited by limiting the number of iterations to fix the computation cost, an effective strategy for real-time simulations. Akin to PBD, our method also works with position updates, but operates directly using the force formulations without converting them to constraints. Parallelization with XPBD is achieved by graph coloring the constraints (i.e. the dual graph) \cite{fratarcangeli_scalable_2015, fratarcangeli_vivace_2016, ton-that_parallel_2023}. However, this dual graph contains multiple times more connections (depending on the types of constraints) than the original graph of vertices, severely limiting the level of parallelism. In comparison, our method is parallelized by coloring the original graph, which leads to much fewer colors (i.e. computation groups that must be processed sequentially) and thereby better parallelism.
%
More importantly, the approximations in XPBD's formulation introduce errors that make it diverge from the solution of implicit Euler and can degrade realism, particularly with large time steps and limited iteration count, which are common in practice. In addition, XPBD particularly struggles with high mass ratios. Our method, on the other hand, has none of these problems.

%Our approach can be seen as a diagonal-block-preconditioned Gauss-Seidel-style descent method for the optimization form of backward Euler. Prior work explored element (can be viewed as a constraint) based Gauss-Seidel methods, e.g. PBD/XPBD \cite{macklin_xpbd_2016, muller2007position}. While there have been substantial efforts to enhance its parallelism \cite{fratarcangeli_scalable_2015, fratarcangeli_vivace_2016, ton-that_parallel_2023}, element-based Gauss-Seidel methods still exhibit fundamental drawbacks. These methods rely on element-based coloring to achieve parallelism, necessitating that elements sharing degrees of freedom do not share the same color. This leads to the formation of a dual graph derived from the mesh's vertex-edge graph, where elements sharing vertices constitute a complete graph. Consequently, the number of colors must be at least as large as the maximum degree among all the vertices. In contrast, our method's parallelism relies on vertex coloring, resulting in nearly one magnitude fewer colors and significantly enhanced parallelism, see \autoref{fig:GraphAndColoring}. Besides parallelism, our method surpasses XPBD in accuracy. XPBD's simplified formulation omits crucial information, which can result in slower convergence and potential loss of realism in certain scenarios, such as large time steps or significant mass ratios. In contrast, VBD successfully handles these challenging cases by leveraging accurate second-order system information, generating plausible results using nearly one-tenth the computational cost of XPBD for complex scenarios, see \autoref{fig:CompareToXPBD_TimeStep}.


In recent years, a growing effort has been placed on accelerating simulations using GPUs  \cite{wang_chebyshev_2015, huthwaite2014accelerated, wang_descent_2016, lan2022penetration, macklin_primaldual_2020, li2020p, li2023subspace}. Among them, the first-order descent methods \cite{wang_descent_2016, macklin_primaldual_2020} have gained popularity due to their excellent parallelism. These methods employ a Jacobi-style preconditioned first-order descent on the backward Euler minimization formulation, enabling full vertex-level parallelization.
%and effectively leveraging the computational power of GPUs. 
However, Jacobi-style iterations typically converge substantially slower than Gauss-Seidel iterations.
%yet they offer superior parallelism. 
Also, such methods necessitate a line search to avoid overshooting and ensure stability.
%In practice, our method converges significantly faster than those first-order descent methods on GPU, which can be attributed to three key factors: our Gauss-Seidel-style iteration, the exceptional stability that eliminates the need for line search, and the local second-order nature of our method. 
%Additionally, choosing Jacobi-style iterations remains cost-effective only in scenarios with abundant parallel computational power, such as when utilizing GPUs for simulations. In contrast, our method also exhibits efficient operation on CPUs, especially for smaller-scale simulations, because it is local second-order descents and it focuses the limited computational power on the more efficient Gauss-Seidel-style iteration. This attribute makes it particularly suitable for applications where the GPU is exclusively reserved for rendering tasks, such as games.

Our method can be categorized as a coordinate descent method for optimization \cite{wright2015coordinate}. In graphics, this technique has been used for geometric processing \cite{naitsat2020adaptive} and simulation with a barrier function \cite{lan_second-order_2023}.  
%Due to the poor parallelism of element coloring, 
Recently, \citet{lan_second-order_2023} proposed a hybrid scheme where Gauss-Sediel and Jacobi iterations are combined at each parallel call.
In comparison, our method uses blocks of coordinates based on vertices instead of blocks based on elements, which results in much better parallelism and smaller local linear systems to solve, leading to faster convergence. 
%In practice, our method converges N magnitudes faster than stencil descent and consumes 2 magnitudes less memory.
%
Concurrently, \citet{yizhou:2024:pbng} present a similar approach to ours for simulating quasistatic hyberelasticity.

\begin{comment}
\subsection{Text from the old introduction}

Physics-based simulation of elastic body dynamics has posed increasing importance in many areas of computer graphics. In numerous scenarios like computer games, telepresence, and training simulators (such as driving or surgical simulators), real-time simulation is essential.  Achieving this demands that every simulation step not only operates within a constrained timeframe but also upholds stability while adhering to a consistently limited time budget.

A well-accepted tool for physics-based simulation is implicit time integration, namely, backward Euler, due to its stability and visual plausibility properties. The solution of Backward Euler can be addressed by linearizing the force formulation and solving a linear system \cite{baraff_large_1998}.
A more recent and popular approach is converting the system to an optimization \cite{martin2011example, gast_optimization_2015}. i.e., variational form, whose extreme point is a valid solution of the Backward Euler. 

The optimization framework employed in this problem allows for the incorporation of classical optimization techniques, facilitating more stable solutions for simulations with larger time steps. For instance, leveraging first-order descent methods.
For example, \citet{wang_descent_2016, macklin_primaldual_2020}  introduced the use of first-order descent methods on GPUs to tackle this optimization problem. These methods are particularly fitting for GPUs due to their inherent parallelism.

Yet, the optimization formulation has drawbacks, notably the varying problem formulation and initial positions in each step. Consequently, achieving consistent convergence within a fixed time budget becomes challenging. Real-time simulators compromise by accepting partially converged results, which visually resemble the final solution. 
However, this compromise can lead to significant visual artifacts (Fig.\ref{}) primarily due to retained residuals from earlier steps. These residuals will accumulate across frames and can jeopardize the solver's stability, potentially resulting in catastrophic simulation failure (\autoref{}). This is because many descent-based methods are known to be unstable under large steps.
%\ziheng{"larger adjustment" and "large step" are a little vague. Are they referring to the same thing as large residual? Do you mean that the initial state is far from the converged state. Maybe we should use a fixed term.} \anka{this is a good point. By "residual" I mean the residual force, which is the gradient of the variational form. By "large step" I mean the initial state is far from the converged state, therefore a larger deformation is required for the model.}

To stabilize simulations affected by accumulated residuals, a common approach involves employing a line search methodology \cite{gast_optimization_2015, wang_descent_2016} to ensure optimization continually reduces energy.
%\ziheng{accumulated residual is only part of the reason why line search is used. A more general case is when the initial state is far from the converged state}
However, the line search method tends to be computationally intensive, particularly due to the reduction operation and intensive GPU-CPU communication, which can be notably slow in GPU implementations. Therefore, a line search is usually the dominant load in the GPU-based implementation. Nevertheless, even when coupled with a line search, these solvers may still encounter failures when the iteration count is limited.

We introduce Vertex Block Descent (VBD), a solver that excels in meeting these criteria: it exhibits superior convergence speed compared to state-of-the-art methods and demonstrates stability even when dealing with substantial residuals carried from preceding steps.
Our method is based on block coordinate descent which performs a vertex-based Gauss-Seidel-style iteration to solve the variantional form of the Backward Euler.
Unlike element-based coloring, our approach involving vertex coloring requires notably fewer colors and a more balanced working load between colors, facilitating highly efficient parallel solutions on both CPU and GPU platforms.  
Remarkably, our method maintains stability even with a fixed step size of 1, eliminating the necessity for line search in most cases. However, if required for specific scenarios, our method only requires a local energy line search to ensure energy descent, which involves only the adjacent tets of each vertex. This process can be executed simultaneously for each vertex, removing the necessity for global reduction.

Comparatively, another popular simulator, XPBD \cite{macklin_xpbd_2016}, is known for its speed and stability under large residuals. However, it struggles with complex material models and excludes essential system information, resulting in slower convergence and potential loss of realism in certain scenarios, such as large time steps or significant mass ratios. In contrast, VBD successfully handles these challenging cases by leveraging accurate second-order system information, ensuring convergence at nearly one-tenth the computational cost of XPBD for complex scenarios.
\end{comment}

==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/03_VertexBlockDescent.tex <==
\section{Vertex Block Descent for Elastic Bodies}
\label{sec:vbd}

Our vertex block descent method is essentially a solver for optimization problems. Therefore, it can be applied to various simulation problems, particularly if they can formulated as an optimization problem.
%
In this section, we explain our method in the context of elastic body dynamics for objects represented by a set of vertices that carry mass and a set of force elements and constraints that act on them. Generalization of our method to other example simulation problems is discussed later in \autoref{sec:othersims}.

%Our vertex block descent method is formulated based on the optimization form of implicit Euler time integration \cite{martin2011example,gast_optimization_2015}. We consider a global system of vertices, each containing position and inertia (i.e. mass and velocity), connected through elements that apply forces, such as FEM elements or springs. Exactly what these vertices and force elements represent depends on the simulated system.

We begin with deriving our global optimization method that splits the simulated system into vertex-level local systems (\autoref{sec:global_opt}). Then, we discuss the methods we use for solving the local systems (\autoref{sec:local_solver}) and describe how we incorporate damping (\autoref{sec:damping}) and constraints (\autoref{sec:constraints}). We present our collision formulation (\autoref{sec:collisions}) and friction formulation (\autoref{sec:friction}). 
%One major advantage of our method is that it produces stable results even when the optimization is not converged in order to fit in a limited computation time budget. For this, 
After explaining our methods for warm-starting our optimization to improve convergence 
%and reduce the residual after bounded computation 
(\autoref{Sec:Initialization}), we describe how to incorporate momentum-based acceleration to improve convergence (\autoref{sec:acceleration}). Finally, we discuss the improved parallelization that our method provides
along with
%and provide some implementation details, including 
methods for efficiently parallelizing dynamically-introduced force elements due to varying collision events (\autoref{sec:parallelism}).
%is the level of parallelism it provides, so we discuss parallelization along with dynamically-changing forces and constraints (\autoref{sec:parallelism}). Finally, we describe how to utilize GPU parallelization to further accelerate our method (\autoref{sec:gpu_implementation}).



\subsection{Global Optimization}
\label{sec:global_opt}

Our vertex block descent method is formulated based on the optimization form of implicit Euler time integration \cite{martin2011example,gast_optimization_2015}.
%
Given a system with $N$ vertices,
we represent the state of our simulation at step $t$ as ($\Vec{x}^t, \Vec{v}^t)$, where $\Vec{x}^t \in  \mathbb{R}^{3N}$ and $\Vec{v}^t\in \mathbb{R}^{3N}$ are the concatenated position and velocity vectors, respectively.
%The well-accepted implicit Euler time integration problem for simulating elastic bodies can be reformulated as the following optimization problem \cite{martin2011example, gast_optimization_2015}:
The resulting optimization problem can be written as
%
\begin{align}
\Vec{x}^{t+1} &= \underset{\Vec{x}}{\operatorname{argmin}} \; G(\Vec{x}) \;,
\end{align}
%
for evaluating the positions at the end of the time step $\Vec{x}^{t+1}$ that minimizes the \emph{variational energy} $G(\Vec{x})$ in the form of
%
\begin{align}
G(\Vec{x}) &= \frac{1}{2h^2} \lVert \Vec{x}-\Vec{y} \rVert _M^2 + E(\Vec{x}) \;.
%\Vec{x^{t+1}} &= \underset{\Vec{x}}{\operatorname{argmin}} \frac{1}{2h^2} \lVert \Vec{x}-\Vec{y} \rVert _M^2 + E(\Vec{x}) \\
%              &= \underset{\Vec{x}}{\operatorname{argmin}} \;  g(x)
\label{Eq:VariantionalFormOfImplicitEuler}
\end{align}
%
The first term here is the \emph{inertia potential}, which contains the time step size $h$,
the mass-weighted norm $\lVert \cdot \rVert_M$, and
%where $h$ is the step size, $\lVert \cdot \rVert_M$ is the mass-weighted norm, $E(\Vec{x})$ is the total potential energy evaluated at $\Vec{x}$, and 
%$\Vec{y}$ is the inertia of the system, such that
%
\begin{align}
\Vec{y} &= \Vec{x}^t + h \Vec{v}^t + h^2 \Vec{a}_{\text{ext}}
\label{Eq:inertia}
\end{align}
%
with a fixed external acceleration $\Vec{a}_{\text{ext}}$, such as gravity. The second term $E(\Vec{x})$ is the \emph{total potential energy} evaluated at $\Vec{x}$.
%represents the constant acceleration caused by external force.

We propose an optimization technique that falls under the category of coordinate descent methods to efficiently minimize this energy $G$.
%We initially 
%Consider a scenario wherein $ E(\Vec{x})$ exclusively represents the contribution from elastic energy.
If we only modify a single vertex at a time, fixing all other vertices, 
%the elastic energy affected is solely from the force elements using this vertex.
the part of the energy term $E(\vec{x})$ that is affected only includes the set of force elements $\mathcal{F}_i$ that are acting on (or using the position of) vertex $i$. Thus, we define the \emph{local variational energy} $G_i$ around vertex $i$ as
%
\begin{align}
    G_i(\Vec{x}) &= \frac{m_i}{2h^2} \lVert \Vec{x}_i-\Vec{y}_i \rVert ^2 + \sum_{j\in \mathcal{F}_i} E_j(\Vec{x}) \;,
     \label{Eq:VBDEnergy}
\end{align}
%
where $m_i$ is the mass of the vertex and $E_j$ is the energy of force element $j$ in $\mathcal{F}_i$.
%denotes the set of all force elements containing vertex $i$.

Note that $G$ is not equal to the sum of local variational energies, i.e. $G(\Vec{x})\neq\sum_i G_i(\Vec{x})$, simply because the force elements appear multiple times in this sum (once for each of its vertices). However, when we modify the position of a single vertex only, the reduction in $G_i$ is equal to the resulting reduction in $G$.

Based on this observation, our method operates on a single vertex at a time and updates its position by minimizing the local energy
%
\begin{align}
\Vec{x}_i &\gets  \underset{\Vec{x}_i}{\operatorname{argmin}} \; G_i(\Vec{x})
\label{eq:position_update}
\end{align}
%
and solves the global system using Gauss-Seidel iterations. Each local minimization for a vertex effectively finds a descent step for $G$ using the degrees of freedom (DoF) for the vertex as a block of coordinates, hence the name \emph{vertex block descent} (VBD).
%
After each iteration, the total reduction in $G$ is equal to the sum of all reductions in $G_i$.
In other words, the energy change of each vertex position adjustment is accumulated to the system energy.
Consequently, if we can make sure that each local energy drops $G_i$ when we are adjusting vertex $i$, we can guarantee that we are descending the system energy $G$.

Thus, our system directly operates on vertex positions 
% (akin to position-based dynamics \cite{muller2007position})
and the resulting velocities are calculated following the implicit Euler formulation
%
\begin{align}
    \Vec{v}^{t+1} = \frac{1}{h}\big(\Vec{x}^{t+1}-\Vec{x}^t\big) \;.
    \label{eq:velocity_update}
\end{align}

%In this case, we can write the optimization in \autoref{Eq:VariantionalFormOfImplicitEuler} for the position of vertex $k$ as
%%optimizing the energy defined by \autoref{Eq:VariantionalFormOfImplicitEuler} is equal to optimizing the local energy $G_k$ of vertex $k$, such that
%
%\begin{align}
%\Vec{x}^{t+1}_k &= \underset{\Vec{x}_k}{\operatorname{argmin}} \; G_k(\Vec{x}) \;,
%\end{align}
%%
%using the local energy $G_k$ that only depends on vertex $k$, such that
%%
%\begin{align}
%G_k(\Vec{x}) &= \frac{m_k}{2h^2} \lVert \Vec{x}_k-\Vec{y}_k \rVert ^2 + \sum_{t\in \mathcal{N}_k} E_t(\Vec{x}) \;,
%%     \Vec{x}^{t+1}_k &= \underset{\Vec{x}_k}{\operatorname{argmin}} \frac{m_k}{2h^2} \lVert \Vec{x}_k-\Vec{y}_k \rVert ^2 + \sum_{t\in \mathcal{N}_k} E_t(\Vec{x}_k) \\
%%                     &= \underset{\Vec{x}}{\operatorname{argmin}} \;  g_k(\Vec{x_k})
%     \label{Eq:VBDEnergy}
%\end{align}
%%
%where $E_t$ is the elastic energy of element $t$ and $\mathcal{N}_k$ denotes the set that includes all force elements containing vertex $k$. In our algorithm, we group the degrees of freedom (DOFs) for each vertex as a block of coordinates and solve this local optimization problem separately, therefore we call our method Vertex Block Descent (VBD).

\subsection{Local System Solver}
\label{sec:local_solver}

The position updates per vertex (in \autoref{eq:position_update}) involve minimizing a local energy that only depends on the position change of a single vertex, represented by $G_i$.
%We can see that \autoref{Eq:VBDEnergy} only has 3 DOFs, 
Note that \autoref{Eq:VBDEnergy} only has 3 DoF, 
so the cost of evaluating and inverting its Hessian is much cheaper compared to the global problem in \autoref{Eq:VariantionalFormOfImplicitEuler}. Therefore, we can fully utilize the second-order information and use Newton's method to minimize the localized energy $G_i$, which involves solving the 3D linear system
\begin{align}
   \Vec{H}_i \, \Delta\Vec{x}_i &= \vec{f}_i \;,
   \label{Eq:VBDLocalSystem}
\end{align}
where $\Delta\vec{x}_i$ is the change in position,
$\vec{f}_i$ is the total force acting on the vertex, calculated using
%
\begin{align}
    \vec{f}_i &= - \frac{\partial G_i(\Vec{x})}{\partial \Vec{x}_i} 
    = - \frac{m_i}{h^2} \left(\vec{x}_i-\vec{y}_i\right) \;- \sum_{j\in\mathcal{F}_i} \frac{\partial E_j(\Vec{x})}{ \partial \Vec{x}_i} \;,
    \label{Eq:VBDForce}
\end{align}
%
and $\Vec{H}_i \in \mathbb{R}^{3 \times 3}$ is the Hessian of $G_i$ with respect to the DoF of vertex $i$, such that
\begin{align}
\Vec{H}_i &= \frac{\partial^2 G_i(\Vec{x})}{\partial \Vec{x}_i \partial \Vec{x}_i} 
    = \frac{m_i}{h^2} \vec{I} \;+ \sum_{j\in\mathcal{F}_i} \frac{\partial^2 E_j(\Vec{x})}{\partial \Vec{x}_i \partial \Vec{x}_i} \;.
    \label{Eq:VBDHessian}
\end{align}
%
%$m_k$ is the mass of vertex $k$.  
%$\frac{\partial^2 G_i}{\partial \Vec{x}_i \partial \Vec{x}_i}$ has two terms: 
Here, the first term is
%the inertia term, which is 
a diagonal matrix and the second one is the sum of Hessians of the
%adjacent tets wrt. 
force elements with respect to
vertex $i$. Intuitively, the solution of this linear system is %trying to find 
the extreme point of the quadratic approximation for the localized energy $G_i$.
%
By reducing $G_i$ with each iteration, we can guarantee a reduction in $G$, thereby iteratively solving the global system in \autoref{Eq:VariantionalFormOfImplicitEuler}.

%Note that $g(\Vec{x}) \neq \sum_k g_k(\Vec{x}_k)$ because the energy of a tet is included by all its vertices' local energy, therefore being counted multiple times in $\sum_k g_k(\Vec{x}_k)$. However, when adjusting each vertex individually, such a property holds:
%\begin{equation}
%\Delta g = \sum_k \Delta g_k
%\label{Eq:VBDStepEnergyChangeProperty}
%\end{equation}
%where $\Delta g$ represents the overall change of  $g(\Vec{x})$ after all the vertices have been changed and $\Delta g_k$ represents the change of the local energy $g_k(\Vec{x}_k)$ after vertex $k$ is adjusted. In other words, the energy change of each vertex adjustment will be accumulated to the system energy. Consequently, if we can make sure that each local energy drops $g_k$ when we are adjusting the corresponding vertex, we can guarantee that we are descending the system energy $g$.



%We use an analytical solver based on Cramer’s law to solve the $3 \times 3$ system given by \autoref{Eq:VBDLocalSystem}, such that
%%
%\begin{align}
% \Delta\Vec{x} &= \frac{1}{\det(\Vec{H}_i)}
% \begin{bmatrix}
%     \det(\Vec{H}_{i,1}) &
%     \det(\Vec{H}_{i,2}) &
%     \det(\Vec{H}_{i,3})
% \end{bmatrix}^T \;,
%\end{align}
%%
%where the matrices $\Vec{H}_{i,c}$ are formed by replacing column $c$ of $\Vec{H}_i$ with the vector $-\partial G_i/\partial\Vec{x}_i$. 
%%\anka{Btw, there is a lot of shared computations in computing$ \det(\Vec{H}_i), \det(\Vec{H}_{i,1}) \det(\Vec{H}_{i,2}),  \det(\Vec{H}_{i,3})$, and our solver exploit this property to save a lot of computations.} \cem{Of course. This is a low-level implementation detail.}


We can analytically solve this system using $\Delta\vec{x}_i=\vec{H}_i^{-1}\vec{f}_i$.
%
For such a small system, the analytical solver is very efficient and stable. We found it to be faster than solvers based on Conjugate Gradient or LU/QR decomposition. 
Another advantage of the analytical solver is that it does not require the Hessian to be positive-definite. Of course, when the Hessian is not positive-definite, the direction given by \autoref{Eq:VBDLocalSystem} may not be a descent direction. Nevertheless, we opt for this direction regardless, recognizing that even when $\Vec{H}_i$ is not positive-definite, solving \autoref{Eq:VBDLocalSystem} still brings us towards the extremum of the quadratic approximation for the localized energy $G_i$.  This solution is close to where the gradient of the inertia and the potential terms balance out and it is usually a stable state of the system. Also, the motivation of the variational form of implicit Euler (\autoref{Eq:VariantionalFormOfImplicitEuler}), is to find a point where ${d G(\Vec{x})/d \Vec{x}=0}$. Therefore, any extreme point is a valid solution of implicit Euler, and it does not have to be a local minimum.
In all our experiments, including those specifically designed stress tests (see \autoref{fig:ExtremeTwist} and \autoref{fig:ExtremeInitialization}), we have consistently observed that this scheme does not pose any issues concerning system stability or convergence.

% \ziheng{It would be clearer to separate the two situations: 1. Hessian not SPD, which is not the issue of the 3x3 solver itself, but an optimization issue (no decrease guarantee). The analytic solver can output a step while other solvers might even fail to generate a step 2. Hessian near singular, analytic solver has a large error.}
An alternative solution to this is the PSD Hessian projection \cite{teran2005robust}. However, it is exceptionally rare for the Hessian to not be positive-definite, and the PSD projection process is notably costly due to multiple SVD decompositions. Engaging in this costly operation to prevent such rare events seems unjustified, especially considering that these occurrences do not jeopardize system stability or convergence significantly.
% \ziheng{this solution only solves not SPD issue but not the near singular issue}

Another challenge with the analytical solver arises when encountering a (nearly) \del{low-rank}\add{rank-deficient} Hessian. 
To address this, we propose a simple solution: if $|\det(\Vec{H}_i)| \leq \epsilon$ for some small threshold $\epsilon$, we opt to bypass adjusting this particular vertex for that iteration. Given that its neighboring vertices are likely to undergo adjustments before the next iteration, it is improbable that its Hessian will remain \del{low-rank}\add{rank-deficient} in subsequent iterations.
With this simple solution, in the extreme scenario where all vertices possess a \del{low-rank}\add{rank-deficient} Hessian, the system could potentially become frozen. Yet, it is crucial to note that such a case is highly improbable, since the Hessian of the inertia potential is always full-rank.
One potential remedy for this would be switching to the modified Conjugate Gradient solver \cite{lan_second-order_2023} when such a case happens. However, doing this will add additional branching to the code and can slow down the solver. Thus, we have not included it in our implementation, but, depending on specific use cases, there is always the flexibility to opt for the Conjugate Gradient solver as a backup solution.




%\subsubsection{Local Linear Search}

The linear system in \autoref{Eq:VBDLocalSystem} corresponds to a single Newton step, so it does not necessarily provide the optimal solution for \autoref{eq:position_update}. In fact, since it is just a second-order approximation of $G_i$, it does not even guarantee a reduction in $G_i$.
%
To ensure the descent of energy with this single step,
%During each VBD step, 
we can incorporate a backtracking line search along the descent direction.
%, ensuring the descent of energy with every step. 
Note that, unlike global line searches in descent-based simulation methods (e.g. \citet{wang_descent_2016}), this line search operates locally. It specifically verifies the descent of $G_i$,
which in turn guarantees a descent in $G$ without the need for evaluating the global system.
%rather than the global energy $G$, eliminating the need for global reductions.
%and CPU-GPU communication in our operations. \cem{we haven't mentioned anything about GPU yet.}

Line search avoids over-shooting and, thereby, ensures stability. 
%However, it involves looping throw all the adjacent tetrahedra, and computing their energy, which means a lot and inconsistent number of random memory access. 
In practice, 
however, the additional computation cost of line search may not be justified. In our experiments,
we found that line search costs an extra 40\% computation time, while not providing any measurable benefits.
%significantly increasing the stability. 
This is because VBD can maintain 
%exceptional 
stability even without line search. 
%Throughout our experiments, we consistently operated without the line search feature and encountered no issues. We provide the option of incorporating the line search for readers, allowing them to implement it according to their specific requirements.
Therefore, the results we present in this paper do not include line search, though it is an option available.
%if needed.


\subsection{Damping}
\label{sec:damping}

Damping plays a crucial role in simulations. It prevents excessive oscillations and also enhances system stability. Despite the inherent numerical damping introduced by the implicit Euler method, providing users with manual control over damping is highly desirable. To address this, we have integrated a simplified Rayleigh damping model into our solver~\cite{sifakis_fem_2012}. This process is both straightforward and efficient, as it also operates locally within the $3 \times 3$ system and utilizes the precomputed stiffness matrix.

Since we are relying on implicit Euler, we can represent the velocity as position change, using $\Vec{v}_i=(\Vec{x}_i-\Vec{x}_i^t)/h$. 
% The damping Hessian is computed as
% \begin{align}
%    \Vec{D}_{i} &= \sum_{j\in\mathcal{F}_i} \frac{k_d}{h} \frac{\partial^2 E_j(\Vec{x})}{\partial \Vec{x}_i \partial \Vec{x}_i} \;,
% \end{align}
Then, we can add the damping term to the Hessian in \autoref{Eq:VBDHessian}, resulting
%
\begin{align}
\Vec{H}_i &= \frac{m_i}{h^2} \vec{I} \;+ \sum_{j\in\mathcal{F}_i} \frac{\partial^2 E_j(\Vec{x})}{\partial \Vec{x}_i \partial \Vec{x}_i} 
    + \left(\sum_{j\in\mathcal{F}_i} \frac{k_d}{h} \frac{\partial^2 E_j(\Vec{x})}{\partial \Vec{x}_i \partial \Vec{x}_i}\right) \;,
    \label{Eq:VBDHessianWithDamping}
\end{align}
%
where $k_d$ is the damping coefficient. Finally, we add the damping 
% Hessian and the damping force to the local system in \autoref{Eq:VBDLocalSystem}, resulting
% %
% \begin{align}
%   \left(\Vec{H}_i + \Vec{D}_{i}\right) \, \Delta\Vec{x}_i &= - \frac{\partial G_i(\Vec{x})}{\partial \Vec{x}_i}    - \Vec{D}_{i}\left(\Vec{x}_i-\Vec{x}_i^t\right) \;.
% \end{align}
force to \autoref{Eq:VBDForce} using the same damping term, such that
%
\begin{align}
    \vec{f}_i &= - \frac{m_i}{h^2} \left(\vec{x}_i-\vec{y}_i\right) -\!\! \sum_{j\in\mathcal{F}_i} \frac{\partial E_j(\Vec{x})}{ \partial \Vec{x}_i}
    - \left(\sum_{j\in\mathcal{F}_i} \frac{k_d}{h} \frac{\partial^2 E_j(\Vec{x})}{\partial \Vec{x}_i \partial \Vec{x}_i}\right)
    \left(\Vec{x}_i-\Vec{x}_i^t\right)
    .
    \label{Eq:VBDForceWithDamping}
\end{align}

%We use this equation instead of \autoref{Eq:VBDLocalSystem} for solving our local system with damping.


\begin{comment}
\cem{Old text to be deleted below:}

Let $\Vec{K}$ be the local $3 \times 3$ stiffness matrix, defined as $\sum_{j\in\mathcal{F}_i} \frac{\partial^2 E_j}{\partial \Vec{x}_i \partial \Vec{x}_i}$ in~\autoref{Eq:VBDHessian}. The damping coefficient, denoted as $\gamma$, is user-defined, controlling the desired damping level.
\ziheng{Optional: In practice, $\Vec{K}$ can be decomposed into distinct parts based on the type of force it corresponds to. Each component, $\Vec{K}_i$, can possess its own damping coefficient. For simplicity, we will focus on demonstrating the implementation of damping for a single stiffness matrix.}
The damping hessian, denoted as $\Vec{H}_d$, is computed as $\gamma \Vec{K}/h$, where $h$ represents the step size. The resulting damping force is given by $-\Vec{H}_d(\Vec{x}_i-\Vec{x}_i^t)$, with the substitution of velocity $\Vec{v}$ by $(\Vec{x}_i-\Vec{x}_i^t)/h$. Subsequently, we modify the linear system~\autoref{Eq:VBDLocalSystem} by incorporating the damping hessian into $\Vec{H}_i$ and adding the damping force to the right-hand side (RHS) to introduce the damping effect.
\end{comment}

    

\subsection{Constraints}
\label{sec:constraints}

Since our method directly manipulates the position of each vertex, managing a constraint on a vertex becomes straightforward. Constraints generally fall into two categories: unilateral ($C(\vec{x}) \leq 0$) or bilateral ($C(\vec{x}) = 0$). With \del{biliteral}\add{bilateral} constraints, if a vertex position is directly set to a specific value, we simply skip updating its position. Otherwise, it is constrained to a (usually linear) subspace. Our approach involves representing the constrained vertex position using the subspace basis. This transforms both the vertex position and gradient into an $L$-dimensional vector, where $L$ is the subspace dimension. Consequently, handling local steps for constrained vertices involves solving an $L\times L$ system.
Regarding unilateral constraints, we allow compromises and define potential energy to be solved alongside other potentials. This method handles world box constraints in our simulations.

%PBD-style soft constraints between vertices can be handled by simply treating them as force elements. Such constraints with infinite stiffness, however, require special treatment, since they generate infinitely strong forces, so simply including them in $\vec{H}_i$ and $\vec{f}_i$ would break the numerical system. 

%Therefore, we suggest first solving \autoref{Eq:VBDLocalSystem} by replacing these infinitely stiff constraints with force elements of high but finite stiffness. This gives VBD a chance to apply position updates towards satisfying these constraints. Finally, to account for infinite stiffness, we can perform a global projection step, which can be expensive, or simply rely on PBD-style updates implemented as a separate pass after completing each iteration by looping over the infinitely stiff constraints. This final step is not included in our tests.



\begin{figure}\vspace{-0.8em}
\centering
\newcommand{\img}[2]{\begin{subfigure}{0.35\linewidth}\centering
\includegraphics[width=\linewidth]{Figures/CollisionPotential/CollisionPotential#1}\vspace{-1.2em}
\caption{#2}\end{subfigure}}
\img{Edge}{Edge-edge}\hspace{0.1\linewidth}%
\img{Triangle}{Vertex-triangle}%
\caption{Two collision types: \sref{a}~edge-edge can have at most two pairs and \sref{b}~vertex-face can have at most one pair with the same color, since vertices on the same side of a collision must have different colors.}
\label{fig:CollisionPotential}
\end{figure}


\subsection{Collisions}
\label{sec:collisions}

Collisions can be handled by simply introducing a quadratic collision energy per vertex, based on the penetration depth $d$, such that
%
\begin{align}
    E_c(\Vec{x}) &= \frac{1}{2} \, k_c \, d^2
    &&\text{with}&
    d &= \max\Big( 0, (\Vec{x}_b - \Vec{x}_a) \cdot \Vec{\hat{n}}\Big) \;,
    \label{eq:collisionEnergy}
\end{align}
%
where $k_c$ is the collision stiffness parameter, $\vec{x}_a$ and $\vec{x}_b$ are the two \emph{contact points} on either side of the collision, and $\vec{\hat{n}}$ is the contact normal.

There are two collision types for triangle meshes (\autoref{fig:CollisionPotential}):
\begin{itemize}
    \item Edge-edge collisions use continuous collision detection (CCD). $\vec{x}_a$ and $\vec{x}_b$ correspond to the intersection points on either edge and the contact normal is the direction between them, i.e. ${\vec{\hat{n}}=\vec{n}/\|\vec{n}\|}$, where ${\vec{n}=\vec{x}_b-\vec{x}_a}$.
    \item Vertex-triangle collisions are detected either by CCD or discrete collision detection (DCD). In this case, $\vec{x}_a$ is the colliding vertex and $\vec{x}_b$ is the corresponding point on either the collision point (for CCD) or the closest point (for DCD) on the triangle \cite{10.1145/3592136}. $\vec{\hat{n}}$ is the surface normal at $\vec{x}_b$.
\end{itemize}

%$\Vec{x}_i$ is the colliding vertex, $\Vec{s}$ is the target position on the surface, and $\Vec{n}$ is the surface normal at $\Vec{s}$. When using continuous collision detection (CCD), $\Vec{s}$ would be the collision point on the surface. With discrete collision detection (DCD), $\Vec{s}$ is the closest point on the surface \cite{10.1145/3592136}.

In our implementation, we perform a DCD at the beginning of the time step using $\vec{x}^t$ to identify vertices that have already penetrated, and the rest of the collisions use CCD.
%
%While we update the vertex positions using Gauss-Seidel iterations, the contact normal $\vec{\hat{n}}$ is computed at the beginning of each iteration and not modified until the next iteration, even though $\vec{x}_a$ and $\vec{x}_b$ are updated sequentially.
We simplify the computation of the gradient and the Hessian of the collision energy by not differentiating through $\vec{\hat{n}}$, i.e. assuming that $\vec{\hat{n}}$ is constant. 

Performing collision detection at every iteration using CCD can be expensive and can easily become the bottleneck. Therefore, in our implementation, we perform CCD once every $n_{\text{col}}$ iterations.
%
While this has the risk of missing some collision events, they are likely to be captured via DCD in the next time step.
%
All detected collisions remain as force elements until the next collision detection.
%
For vertex-triangle collisions detected with DCD, it is important to recompute the closest point ($\vec{x}_b$) before computing the gradient and Hessian of $E_c$.

%In our tests, we set $k_c$ as the largest material stiffness in the system.

%In our implementation, we use a combination of CCD and DCD, and a quadratic collision energy based on the penetration depth:
%\begin{equation}
%    E_c = \frac{1}{2} \, k \, \big( (\Vec{x}_i - \Vec{s}) \cdot \Vec{n}\big)^2
%\end{equation}
%where $k$ is the collision stiffness, $\Vec{x}_i$ is the position of the penetrating vertex, $\Vec{s}$ is the closest surface point computed by \cite{10.1145/3592136} for DCD collisions, or the colliding point for CCD collisions and $\Vec{n}$ is the surface normal at $\Vec{s}$. We perform a DCD at the beginning of the time step to identify the already penetrated vertices and the rest of the collisions are detected by CCD. 



\subsection{Friction}
\label{sec:friction}

%VBD allows applying friction to colliding vertices in various ways. Let $\vec{x}_a$ and $\vec{x}_b$ represent \emph{contact points} on two sides of a detected collision (for a vertex-triangle collision, one is the colliding vertex and the other is the corresponding point on the triangle, and for an edge-edge collision, they are the closest points on the two edges).

%We start by computing the relative translation between the two sides. Say $\vec{x}_a$ and $\vec{x}_b$ is the \textit{contact points} of the two sides,  specifically being the vertex and the closest (or colliding point, in case of continuous collision detection) point on the face in case of vertex-face collision, and the closet points to each other in case of edge-edge collisions. $\vec{x}_i, i=1,2,3,4$ are the 4 vertices involved in this collision, and $\vec{x}_a$ and $\vec{x}_b$ are linear combination of those 4 vertices. 

To compute friction for collision $c$, we must consider the relative motion of the contact points defined as
%We adopt the friction model of \emph{incremental potential contact} (IPC)~\cite{li2020incremental}.
%The relative translation can be computed as:
\begin{equation}
    \delta\vec{x}_c  = \big(\vec{x}_a - \vec{x}_a^t\big) - \big(\vec{x}_b - \vec{x}_b^t\big) \;,
\end{equation}
where $\vec{x}_a^t$ and $\vec{x}_b^t$ are the positions of $\vec{x}_a$ and $\vec{x}_b$ at the beginning of the time step.
%, which can be computed through interpolating $\vec{x}_1^t, \vec{x}_2^t, \vec{x}_3^t, \vec{x}_4^t$ using the same ratio.

With this $\delta\vec{x}_c$, we can use the friction model of \emph{incremental potential contact} (IPC)~\cite{li2020incremental}.
First, we project $\delta\vec{x}_c$ to the 2D contact tangential space,
using a transformation matrix $\vec{T}_c \in \mathbb{R}^{3 \times 2}$, to evaluate the tangential relative translation $\vec{u}_c=\Vec{T}_c^T\delta\Vec{x}_c$, where $\vec{T}_c=[\vec{\hat{t}}~\vec{\hat{b}}]$ is formed by a tangent $\vec{\hat{t}}$ and binormal $\vec{\hat{b}}$ vectors orthogonal to $\vec{\hat{n}}$.
%which is orthogonal to the contact normal ($\vec{\hat{n}}$ in \autoref{eq:collisionEnergy}), obtaining the tangential relative translation $\Vec{u}$. Such that $\Vec{u}=\Vec{T}^T\delta\Vec{x}$, where $\Vec{T} \in \mathbb{R}^{3 \times 2}$ is the projection matrix, whose 2 columns are the 2 orthogonal-normal basis of the contact tangential space,  such that $\vec{T}^T\vec{T}=I_2$.
The signed magnitude of the collision force applied on vertex $i$ is $\lambda_{c,i}=\frac{\partial E_c}{\partial \Vec{x}_i}\cdot \vec{\hat{n}}$. Note that the sign of $\lambda_{c,i}$ is different for vertices on different sides of the collision.
Let $\mu_c$ be the friction coefficient. We can then calculate the friction force using
\begin{align}
   %F(\Vec{x_i}, \lambda_i, \Vec{T}) 
   \vec{f}_{c,i}
   &= -\mu_c\,\lambda_{c,i}\,\frac{\partial \delta \Vec{x}_c}{\partial \Vec{x}_i}\,\Vec{T}_c\,f_1(\|\Vec{u}_c\|)\frac{\Vec{u}_c}{\|\Vec{u}_c\|}\;\text{,  where} \\
   f_1(u) &=
    \begin{cases}
      2\left(\frac{u}{\epsilon_vh}\right) - 
       \left(\frac{u}{\epsilon_vh}\right)^2, &u \in (0,h\epsilon_v)\\
      1, &u \geq h\epsilon_v
    \end{cases}.
   \label{Eq:IPC_friction}
\end{align}
Here, $f_1$ serves as a smooth transition function between static and dynamic friction. 
When the relative velocity exceeds a small threshold $\epsilon_v$, dynamic friction is applied. Conversely, if the relative velocity is below this threshold, static friction is applied, scaling between the range of $[0,1]$. 
% The incorporation of this smooth transition allows us to compute the corresponding Hessian and seamlessly integrate friction into our solver.

In our formulation, we need the Hessian of the friction term, which is the derivative of this function. We approximate the derivative by not differentiating through $\|\Vec{u}_c\|$ for a more stable friction force formulation \cite{macklin_primaldual_2020}, such that
%We further provide a simplified Hessian of the friction term:
\begin{align}
\frac{\partial \vec{f}_{c,i}}{\partial \vec{x}_i} &\approx -\mu_c\,\lambda_{c,i}\,\frac{\partial \delta\vec{x}_c}{\partial \vec{x}_i}\,\Vec{T}_c\,\frac{f_1(\|\Vec{u}_c\|)}{\|\Vec{u}_c\|} \Vec{T}_c^T\,  \left(\frac{\partial \delta\vec{x}_c}{\partial \vec{x}_i}\right)^T\;.
\end{align}
%Note that here we do not differentiate through $\|\Vec{u}_c\|$. This is suggested by \cite{macklin_primaldual_2020}, as it can make the friction model stable. 
Without this approximation, PSD projection and line search might be needed to ensure stability.
%The friction is solved by suming $F(\Vec{x_i}, \lambda, \Vec{T})$ to the right hand side of \autoref{Eq:VBDLocalSystem} and suming $\frac{\partial F(\Vec{x_i}, \lambda_i, \Vec{T})}{\partial\Vec{x}_i}$ to $\vec{H}_i$.
%Note that we use $\Vec{T}$ and $\lambda_i$ from the previous iteration as IPC did so that they are treated as constant variables during the hessian calculation.
Finally, all friction forces $\vec{f}_{c,i}$ and their derivatives $\partial \vec{f}_{c,i}/\partial\vec{x}_i$ are added to $\vec{f}_i$ and $\vec{H}_i$, respectively.
% $\Vec{T}_c$ and $\lambda_{c,i}$ are computed at the beginning of adjusting each color, prior to updating any of the colliding vertices.

\begin{comment}
    
While the computational cost of friction itself is negligible, it could potentially impact the overall system's stability and convergence. Particularly in the earlier iterations when the system can be far from convergence, the friction force can become exceedingly large, resulting in a highly stiff system, which can lead to instabilities due to overshooting, requiring line search. To mitigate this issue, IPC applies friction only during the last few iterations when the system approaches convergence. This solution can also be implemented in VBD; however, it necessitates either more iterations or smaller timesteps and requires a mechanism to assess convergence. In real-time simulations prioritizing speed, a fixed and small number of iterations is often preferred. Therefore, in such cases, we fall back to a %direct modification of relative velocities. 
simple alternative friction model described below.

Our simple friction model is \emph{velocity adjustment} that only modifies velocities at the end of each timestep by replacing \autoref{eq:velocity_update} with
%
\begin{align}
    \Vec{v}_i^{t+1} = \frac{1}{h}\left(\Vec{x}^{t+1}_i-\Vec{x}^t_i 
    - \sum_{c\in\mathcal{C}_i} 
    \vec{T}_c\Vec{u}_c\,f_{c,i}(\|\Vec{u}_c\|) \right) \;,
\end{align}
%
where $\mathcal{C}_i$ is the set of collisions for vertex $i$ and $f_{c,i}$ is a clamping function, such that
%
\begin{align}
\cem{Are we keeping this?}
    f_{c,i}(u) = \begin{cases}
      \frac{\mu\,\lambda_{c,i}}{u\,m_i}\;, & \text{if } 
       \frac{\mu\,\lambda_{c,i}}{u\,m_i} < \frac{1}{2} \\
      \frac{1}{2}\;, & \text{otherwise.}
    \end{cases}  
\end{align}
%
Here, $f_{c,i}$ ensures that the velocity change due to friction does not exceed the relative motion. Since velocity adjustment only impacts the velocities transferred to the next time step, it does not impact the stability of the system. However, it lacks the quality of the friction force model and cannot properly handle static friction.

Depending on specific use cases, implementations of VBD can choose between these two friction models, as needed.
\end{comment}


\begin{comment}


\subsubsection{\cem{old simple friction text}}

The relative velocities modification is applied after all the iterations have been completed. 
Similarly, for each colliding point $i$, we compute $\vec{u}$ and the collision force $\lambda_i$ using the vertex positions after iteration. The relative velocity can be computed as $\delta \Vec{v} = \vec{u}/h$. Our approach operates directly on $\delta \Vec{v}$'s norm, updating it to be:
\begin{align}
    l = 
    \begin{cases}
      |\delta \Vec{v}| - h \mu \lambda_i / m_i & \text{if } |\delta \Vec{v} - h \mu \lambda_i / m_i > 0.5 |\Tilde{\vec{v}}_i| \\
       0.5 |\delta \Vec{v}|& \text{otherwise}
    \end{cases}  
\end{align}
and we update vertex $i$'s velocity as:
\begin{equation}
    \vec{v}_i^{\text{new}} = \vec{v}_i + \vec{T}\delta \Vec{v}\frac{ (l - |\delta \Vec{v}|)}{|\delta \Vec{v}|}
\end{equation}
The inclusion of the 0.5 ratio ensures that the relative velocity is, at most, changed to 0, preventing it from being reversed. 
This process is applied in a Jacobi-style manner, where all vertices are processed together. For vertices involved in multiple collisions, the process is sequentially executed for each collision.
We acknowledge this is merely a crude approximation of friction, addressing the repulsive part of the contact force separately in the variational form and subsequently applying the frictional force based on a forward integration, which may present challenges in accurately representing static friction.
Depending on specific use cases, implementations of VBD can choose between these two friction models, as needed.

\subsubsection{\cem{old friction section}}
Friction represents another pivotal factor affecting the authenticity of physical simulations. Instead of directly modifying positions or velocities (as done in XPBD and Projective Dynamics for handling friction), we adopt the friction model of \emph{incremental potential contact} (IPC)~\cite{li2020incremental}. Though we use different collision forces, the friction formulation is identical. This friction model offers two significant advantages. Firstly, it adheres to Coulomb's law of friction, enhancing the realism of the simulation. Second, in line with IPC, we employ a smoothed friction function that facilitates a smooth transition from dynamic friction to static friction. This approach allows us to differentiate the frictional gradient and seamlessly integrate it into our solver.


\cem{Please add the math to describe how friction is implemented.}
\cem{We don't have to explain why this friction model works, but we should provide sufficient information for the reader to implement it in VBD.}
We will present the formulas for a single point-triangle collision pair here and direct readers to the IPC paper for a more in-depth understanding.
We use the colliding triangle as the tangent plane. By interpolating the displacements of the triangle's three vertices, we can compute the approximated displacement of the triangle and the relative displacement between the vertex and triangle, denoted by $\Vec{u}$.
Note that $\Vec{u}$ is a 2d vector defined on the tangent plane.
The mapping from displacement $\Vec{x}-\Vec{x}_n$ to $\Vec{u}$ is linear and we define this mapping as $\Vec{T}(\Vec{x}) \in \mathbb{R}^{3n \times 2}$ such that $\Vec{u}=\Vec{T}(\Vec{x})^T(\Vec{x}-\Vec{x}_n)$.
%Let $\Vec{T}(\Vec{x}) \in \mathbb{R}^{3n \times 2}$ be the sliding basis for the collision \cem{Where does this $\Vec{T}(\Vec{x})$ come from? How can I calculate it?} and $\Vec{u} \in \mathbb{R}^{2}$ be the local relative sliding displacement, given by $\Vec{u}=\Vec{T}(\Vec{x})^T(\Vec{x}-\Vec{x}_n)$.
 Let $\mu$ be the friction coefficient and $\lambda$ be the magnitude of collision force. 
Then we have frictional force:
\begin{align}
   F(\Vec{x}, \lambda, \Vec{T}) &= -\mu\lambda\Vec{T}(\Vec{x})f_1(\|\Vec{u}\|)\frac{\Vec{u}}{\|\Vec{u}\|}\text{,  where} \\
   f_1(u) &=
    \begin{cases}
      -\frac{u^2}{\epsilon^2_vh^2}+\frac{2u}{\epsilon_vh}, &u \in (0,h\epsilon_v)\\
      1, &u \geq h\epsilon_v
    \end{cases}.
   \label{Eq:IPC_friction}
\end{align}
$f_1$ serves as a smooth transition function between static and dynamic friction. When the relative velocity exceeds a small threshold $\epsilon_v$, dynamic friction is applied. Conversely, if the relative velocity is below this threshold, static friction is applied, scaling between the range of $[0,1]$. The incorporation of this smooth transition allows us to compute the corresponding hessian and seamlessly integrate friction into our solver.

While the computational cost of friction itself is negligible, it could potentially impact the overall system's stability and convergence. Particularly when the system is far from converging, the friction force can become exceedingly large, resulting in a highly stiff system and the potential for overshooting. To mitigate this issue, IPC applies friction only during the last few iterations when the system approaches convergence. This solution can also be implemented in VBD; however, it necessitates either more iterations or smaller timesteps and requires a mechanism to assess convergence. In real-time simulations prioritizing speed, a fixed, small number of iterations is often preferred. Therefore, in such cases, we fall back to direct modification of relative velocities. 
\cem{How is this done? Please be specific with math. Is this the same as XPBD?} 
This method is applied after all the iterations have been completed. For each colliding vertex $i$, the procedure starts by computing the relative velocity to the other side of the collision. \cem{This is a bit ambiguous. We can be more specific about how to compute the relative velocity.} Subsequently, this velocity is projected onto the contact tangential plane to obtain its tangential component, denoted as  $\Tilde{\vec{v}}_i$. The collision force $\vec{f}_c$ is then computed based on the positions after the iterations. \cem{how is $\vec{f}_c$ computed?}  Then we update this tangential relative velocity's
norm as:
\begin{align}
    l = 
    \begin{cases}
      |\Tilde{\vec{v}}_i| - h \gamma_f |\vec{f}_c| / m_i & \text{if } |\Tilde{\vec{v}}_i| - h \gamma_f |\vec{f}_c| / m_i > 0.5 |\Tilde{\vec{v}}_i| \\
       0.5 |\Tilde{\vec{v}}_i|& \text{otherwise}
    \end{cases}  
\end{align}
where $\gamma_f$ is the friction ratio. \cem{is this the ``friction coefficient''?} \anka{yes.}
The inclusion of the 0.5 ratio ensures that the relative velocity is, at most, changed to 0, preventing it from being reversed. 
This process is applied in a Jacobi-style manner, where all vertices are processed together. For vertices involved in multiple collisions, the process is sequentially executed for each collision.
We acknowledge this is merely a crude approximation of friction, addressing the repulsive part of the contact force separately in the variational form and subsequently applying the frictional force based on a forward integration, which may present challenges in accurately representing static friction.
Depending on specific use cases, implementations of VBD can choose between these two friction models, as needed.

\end{comment}


\subsection{Initialization}
\label{Sec:Initialization}

%Using optimization formulation allows for flexible initialization. Typically, if the simulation converges, different initializations shouldn't significantly affect the final results, except for their impact on convergence speed. However, when the convergence is not guaranteed due to limited computational time, initialization gains importance. A better initialization can guide the simulation closer to the actual solution. We explore various schemes: initializing from the previous position or inertia. 

Since our method is an iterative solver, we begin with an \emph{initial guess} for $\Vec{x}$. The closer this initial guess is to the resulting $\Vec{x}^{t+1}$, the fewer number of iterations we would need to converge. 
\del{Regardless of the initialization strategy for determining this initial guess, because we are solving an optimization problem, the system is expected to converge to  result, though it may require a different number of iterations.}\add{Typically, if the simulation converges, different initializations should not significantly affect the final results, although they may influence the number of iterations required to achieve convergence. }

%This initial guess can be simply the positions at the end of the previous step (i.e. $\Vec{x}=\Vec{x}^t$), but it does not have to be.

Providing a good initial guess (one that is close to $\Vec{x}^{t+1}$) is particularly important for applications with a limited computation budget, e.g. using a fixed number of iterations. In such applications, the initial guess can strongly impact the remaining residual at the end of the final iteration.


\begin{figure}
\centering
\includegraphics[width=\linewidth,trim=0 0 0 0, clip]{Figures/AdaptiveInitialization/D4}
\newcommand{\scap}[2]{\begin{subfigure}{0.2\linewidth}\caption{#2}\label{fig:Initialization:#1}\end{subfigure}}
\scap{a}{Previous\\\hspace*{1em}position}\hfill%
\scap{b}{Inertia\\~}\hfill%
\scap{c}{Inertia \& acceleration}\hfill%
\scap{d}{\textbf{Adaptive}\\~}\hfill%
\scap{e}{Reference\\~}
\caption{Different initialization options for a swinging elastic pendulum dropped from the same height (blue line) simulated with our method using only 20 iterations per frame, showing the same frame of the simulation. Notice that initializing using \sref{a}~previous position and \sref{b}~inertia fail to properly move under gravity, while \sref{c}~inertia and acceleration leads to accessive stretching (red line) when VBD does not run to convergence. \sref{d}~Our adaptive solution closely matches \sref{e}~the reference generated by fully converged Newton's method (green line).}
\label{fig:Initialization}
\end{figure}


We begin with considering three simple options for initialization: %starting with no motion or no force element:
%\begin{enumerate}
%    \item \textbf{Previous position:} $\Vec{x}=\Vec{x}^t$
%    \item \textbf{Full inertia:} $\Vec{x}=\Vec{y}$
%\end{enumerate}
\begin{align*}
    \text{(a)~}&\text{\textbf{Previous position:}}&
    \Vec{x} &= \Vec{x}^t \\%&\hspace{5em}\\
    \text{(b)~}&\text{\textbf{Inertia:}}&
    \Vec{x} &= \Vec{x}^t + h\vec{v}^t \\%&\hspace{5em}\\
    \text{(c)~}&\text{\textbf{Inertia and acceleration:}}&
    \Vec{x} &= \vec{x}^t + h\vec{v}^t + h^2\vec{a}_{\text{ext}} = \Vec{y}
\end{align*}

Option (a) struggles with substantially stiff materials. As we adjust each vertex separately, assuming the others remain fixed, our method must lean on the inertia potential's gradient (i.e. ${m_i(\vec{x}_i-\vec{y}_i)/2h^2}$) to march toward the local minimum. With stiff materials, this method results in notably slower convergence rates due to the inertia potential being considerably less stiff. Consequently, it encounters challenges in simulating scenarios that resemble free fall, like a swinging elastic pendulum at its maximum height, as shown in \autoref{fig:Initialization:a}.

Option (b) allows the system to start with the inertia of the previous step, which helps, but terminating the iterations prior to convergence can again result in local material stiffness overpowering external acceleration, as shown in \autoref{fig:Initialization:b}.

Option (c) is similar to the initialization of position-based dynamics, and performs notably better as it effectively preserves inertia and properly reacts to external acceleration.
%and yields visually realistic outcomes
%However, when the optimization does not converge, it often fails to properly represent the material's stiffness, resulting in overstretching. 
However, with a limited number of iterations, materials behave softer than they should, often resulting in overstretching or collapsing under gravity.
An example of this can be seen in \autoref{fig:Initialization:c}, where the pendulum extends more than it should.
Most notably, it struggles with steady objects at rest in contact, consistently initializing them into a penetrating state, as if they are in free fall. In such cases, the contact forces must entirely undo the position change of initialization during the iterations. This not only creates unnecessary computation, but also places considerable strain on the accuracy of the collision detection and handling methods (including friction). Therefore, properly simulating objects that are stacked on top of each other becomes a major challenge with this initialization option.

%An even more critical issue arises as it struggles to simulate a completely static object, consistently initiating material in a free-falling state. This limitation significantly impacts simulating object stacking, requiring objects to penetrate and recover even when they have come to a complete stop. Consequently, this places considerable strain on collision detection and handling methods.



\begin{figure}
\centering
%\includegraphics[width=\columnwidth]{Figures/10_2SquishyballColliding.pdf}
% \newcommand{\fig}[1]{\includegraphics[width=0.33\linewidth,trim=700 100 640 400, clip]{Figures/AdaptiveInitialization/#1}}
% \fig{A}\hfill%
% \fig{B}\hfill%
% \fig{V}\hfill%
% \includegraphics[width=0.2092\linewidth,trim=0 0 0 0, clip]{Figures/AdaptiveInitialization/a}\hfill%
% \includegraphics[width=0.2092\linewidth,trim=0 0 0 0, clip]{Figures/AdaptiveInitialization/b}\hfill%
% \includegraphics[width=0.126\linewidth,trim=0 0 0 0, clip]{Figures/AdaptiveInitialization/c}\hfill%
% \includegraphics[width=0.22\linewidth,trim=0 0 0 0, clip]
% {Figures/AdaptiveInitialization/d}
% \includegraphics[width=0.224\linewidth,trim=0 0 0 0, clip]
% {Figures/AdaptiveInitialization/e}
% \includegraphics[width=\linewidth,trim=0 100 0 0, clip]{Figures/AdaptiveInitialization/D2}\vspace{-1.6em}
% \scap{previous position}{0.3}%
% \scap{full inertia}{0.233}%
% \scap{adaptive}{0.233}%
% \scap{reference}{0.233}%
% \vspace{0.2em}
% \newcommand{\scap}[2]{\begin{minipage}{#2\linewidth}~\small{#1}\end{minipage}}
% \includegraphics[width=0.9\linewidth,trim=220 150 220 50, clip]{Figures/AdaptiveInitialization/abc}
\newcommand{\spc}{~\vspace{0.2em}}
\includegraphics[width=\linewidth,trim=0 0 0 0, clip]{Figures/AdaptiveInitialization/combined3}\vspace{-0.34\linewidth}\\
\begin{flushright}\small 
1.0\spc\\
0.8\spc\\
0.6\spc\\
0.4\spc\\
0.2\spc\\
0.0\spc\\
gravity initialization factor ($\tilde{a}$)
\end{flushright}
\caption{The ratio of gravity $\tilde{a}$ used with adaptive initialization during the swinging of an elastic pendulum. The model is a single-piece tetrahedral mesh. It automatically distinguishes vertices in approximate free-fall (red) and those where elasticity counteracts gravity (blue).}
\label{fig:AdaptiveInitialization}
\end{figure}


We propose an adaptive initialization scheme that combines options (b) and (c), taking advantage of the freedom that VBD provides in the choice of initialization.
%that takes advantage of this flexibility of initialization. 
This scheme uses
%
\begin{align*}
    \text{(d)~}&\text{\textbf{Adaptive:}}&
    \Vec{x} &= \vec{x}^t + h\vec{v}^t + h^2\vec{\tilde{a}}
    &\hspace{0.2\linewidth}
\end{align*}
%
replacing the external acceleration $\vec{a}_{\text{ext}}$ in (c) with an estimated acceleration term $\vec{\tilde{a}}$, determined by exploiting the typical similarity between two consecutive time steps.
%The inertia term consists of a velocity term and a constant acceleration term, with acceleration often proving more significant due to its independence from the simulation state. Typically, gravity constitutes the dominant component of this constant acceleration. 
%Our approach centers on a specific treatment of gravitational acceleration. 
We begin with the acceleration of the previous frame
%By deriving an estimated acceleration $\Vec{\tilde{a}}^{t+1}$ from the velocity of the past two steps, such that 
${\Vec{a}^t=(\vec{v}^t-\vec{v}^{t-1})/h}$ and compute its component $a^t_{\text{ext}}$ along the external acceleration direction ${\vec{\hat{a}}_{\text{ext}}=\vec{a}_{\text{ext}}/\|\vec{a}_{\text{ext}}\|}$, such that ${a^t_{\text{ext}}=\vec{a}^t\cdot\vec{\hat{a}}_{\text{ext}}}$.
%$\Vec{a}_k$'s component aligned with the direction of gravity. 
Then, we simply make sure that the estimated acceleration does
%clamp the norm of this component to 
not exceed the external acceleration, using
%gravitational acceleration $\vec{g}$:
\begin{align}
    \vec{\tilde{a}} &= \tilde{a}\,\vec{a}_{\text{ext}} \;, &&\text{where}&
    \tilde{a} &=
    \begin{cases}
      1\;, & \text{if $a^t_{\text{ext}}>\|\vec{a}_{\text{ext}}\|$}\\
      0\;, & \text{if $a^t_{\text{ext}}<0$}\\
      a^t_{\text{ext}}/\|\vec{a}_{\text{ext}}\|\;, & \text{otherwise.}
    \end{cases}       
\end{align}
%We replace each vertex' constant acceleration in \autoref{Eq:inertia} with $\Tilde{\vec{a}}_k$ to compute the initialization position (the inertia term is still computed using  $\Vec{a}_{ext}$). This initialization also works for the other external force that is already known before the simulation starts.
%In practice, this approach effectively prevents overstretching and maintains the static state of objects.
This adaptive approach includes external acceleration in the initialization when the motion of a vertex resembles free fall. When an object is stationary, however, as in rest-in-contact, it maintains the previous position in the initialization, preventing undesired penetrations before the first iteration. It also successfully avoids excessive stretching, as can be seen in \autoref{fig:Initialization:d}. Visualizations of different $\tilde{a}$ values in this simulation are shown in \autoref{fig:AdaptiveInitialization}. In short, our adaptive initialization is a simple but effective strategy and it is possible because VBD does not dictate a particular initialization (unlike XPBD, for example).






%\subsection{Momentum-Based Acceleration}
\subsection{Accelerated Iterations}
\label{sec:acceleration}

We use the Chebyshev semi-iterative approach \cite{wang_chebyshev_2015} to improve the convergence of our method, though other momentum-based acceleration techniques, such as the Nesterov’s method \cite{golub2013matrix} can be applied as well.
The Chebyshev method
%Momentum-based acceleration techniques, such as the Chebyshev semi-iterative method \cite{golub2013matrix} or the Nesterov’s method \cite{golub2013matrix} can be incorporated to improve the convergence of our method. We use the Chebyshev semi-iterative approach \cite{wang_chebyshev_2015} as our accelerator, which 
iteratively computes an acceleration ratio based on the approximation of the system's spectral radius. Instead of directly using the output vertex positions of Gauss-Seidel ${\vec{\bar{x}}}^{(n)}$ after iteration $n$, it recomputes the positions at the end of the iteration
using
\begin{align}
    \vec{x}^{(n)} &= \omega_{n} ({\vec{\bar{x}}}^{(n)} - \vec{x}^{(n-2)} ) + \vec{x}^{(n-2)} \;,
    \label{eq:accelerator}
\end{align}
where 
%$\vec{x}^{(n)}$ is the vertex positions after iteration $n$, $\hat{\vec{x}}^{(n)}$ is the positions prior to acceleration, right after the Gauss-Seidel iteration, and 
$\omega_{n}$ is the acceleration ratio that changes at each iteration as
\begin{align}
    \omega_{n}&=\frac{4}{4-\rho^2\omega_{n-1}}
    &\text{with}&&
    \omega_1 &= 1
    &\text{and}&&
    \omega_2 &= \frac{2}{2-\rho^2} \;,
\end{align}
%give given the initial conditions $\omega_1=1$ and $\omega_2=\frac{2}{2-\rho^2}$. 
where $\rho \in(0,1)$ is the estimated spectral radius, which can be set manually, or automatically tuned using the technique introduced in \cite{wang_descent_2016}.
Note that this position recomputation procedure is performed globally after each Gauss-Seidel iteration is completed, 
%i.e., after all the colors have been swept, not simultaneously with each local step.
not after each local solver step.



\begin{figure}
\centering
\newcommand{\figA}[3]{\begin{subfigure}{0.315\linewidth}\centering
\includegraphics[width=\linewidth,trim=450 300 550 50,clip]{Figures/AccelerationComparison/#1}
\caption{#2}\label{fig:AccelerationComparison:#3}
\end{subfigure}}
\begin{subfigure}{0.36\linewidth}\centering
\includegraphics[width=\linewidth,trim=450 200 450 150,clip]{Figures/AccelerationComparison/a}
\caption{Not accelerated}\label{fig:AccelerationComparison:a} 
\end{subfigure}\hfill%
\figA{b}{Accelerated}{b} \hfill%
\figA{c}{Reference}{c} 
\caption{
Demonstrating the accelerator's impact in a collision-intensive scene: a squishy ball (230K vertices, 700K tetrahedra) dropping and bouncing. Both \sref{a} and \sref{b} use $h=1/120\text{ seconds}$ with a constant number of $120$ iterations per time step, taking $0.11\text{ seconds}$ of average computation time per frame. \sref{a}~Without acceleration 120 iterations appear to be insufficient. \sref{b}~Our acceleration scheme ($\rho=0.95$), skipping colliding vertices, manages to resolve complex collisions, notably enhancing elasticity convergence for much stiffer outcomes, 
%compared to results with no acceleration.
closely matching \sref{c}~the reference computed using 2000 iterations.}
\label{fig:AccelerationComparison}
\end{figure}




This accelerator was originally developed for solving linear systems, assuming the energy to be smooth and (nearly) quadratic. Elastic energy generally fulfills these criteria. However, collision energy tends to be discontinuous and highly stiff, making the use of an accelerator in collision-intensive scenes prone to overshot and compromise the system's stability. To address this, we propose a simple yet highly effective solution for accelerating scenes with collisions: skipping the accelerations for actively colliding vertices. 
Note that the acceleration must be a continuous process. If a vertex is detected colliding at a certain iteration, we will skip the acceleration for it in all the following iterations in the same step, regardless of whether the collision has been resolved. 
This approach has minimal impact on the convergence of elasticity, since 
%colliding vertices typically constitute less than 1\% of the total. 
typically only a small fraction of vertices are in collision.
Also, for those colliding vertices, the elasticity is usually overpowered by the collision forces.
Thus, this solution maintains the stability of the system, while effectively accelerating the convergence of elasticity, as shown in \autoref{fig:AccelerationComparison}.





\subsection{Parallelization}
\label{sec:parallelism}

Gauss-Seidel-type iterative methods are often parallelized using graph coloring by determining groups (i.e. colors) that can be handled in parallel without impacting the sequential nature of the Gauss-Seidel loop. Obviously, the same can be applied to VBD by simply coloring vertices such that no force element uses multiple vertices of the same color.


\begin{figure}
\centering
\newcommand{\figWithWidth}[3]{\begin{subfigure}{0.495\linewidth}\centering
\includegraphics[width=0.8\linewidth]{Figures/GraphAndColoring/GraphAndColoring#3}\vspace{-0.5em}
\caption{#2}\label{fig:GraphAndColoring:#1}
\end{subfigure}}
\newcommand{\figA}[3]{\begin{subfigure}{0.495\linewidth}\centering
\includegraphics[width=\linewidth,trim=0 240 0 0,clip]{Figures/GraphAndColoring/#3}\vspace{-0.5em}
\caption{#2}\label{fig:GraphAndColoring:#1}
\end{subfigure}}
\figWithWidth{a}{Vertex colors: 3}{Verts}\hfill%
\figWithWidth{b}{Dual graph \& element colors: 8}{Elems}
\figA{c}{Vertex colors: 8}{Vert}\hfill%
\figA{d}{Element colors: 76}{Tet}
\caption{Coloring vertices vs. elements: \sref{a}~vertex coloring needs 3 colors for 10 vertices while \sref{b}~element coloring (i.e. coloring the vertices of the dual graph) needs 8 colors for 10 triangles in this example. The difference is more pronounced for tet-meshes: \sref{c}~our vertex coloring uses only 8 colors for 3,891 vertices while \sref{d}~our element coloring implementation needs 76 colors for 14,802 tetrahedra in this example.
%In the context of a triangular mesh, vertex coloring relies on the vertex-edge graph (a), while the element is based on the dual graph (b), where the nodes represent the elements. In the latter case, a vertex with 7 neighboring triangles transforms into a 7-complete graph. An illustrative example involves the coloring of an octopus model using \cite{pereira2005register}, wherein 8 colors are needed for vertex coloring, and 76 colors are required for tetrahedron coloring. The distribution of the number of vertices and tetrahedra for each color is also depicted in (c) and (d), respectively.
}
\label{fig:GraphAndColoring}
\end{figure}

%\begin{figure}
%\centering
%\newcommand{\figB}[2]{\begin{subfigure}{0.495\linewidth}\centering
%\includegraphics[width=\linewidth,trim=0 10 64 50,clip]{Figures/GraphAndColoring/#1}
%\caption{#2}\label{fig:LoadEquilibrium:#1}
%\end{subfigure}}
%\figB{e}{combining 2 models}
%\figB{f}{combining 4 models}
%\caption{Our computational load equilibrium algorithm's outcomes for 2 and 4 octopus models (same as the model in \autoref{fig:GraphAndColoring}:c)  respectively, respectively. Each color in the bar chart represents a model. After the equilibrium, the ratio between the largest and smallest color became 1.39 for 2 models and 1.25 for 4 models, as opposed to 70 for a single model.}
%\label{fig:LoadEquilibrium}
%\end{figure}


The advantage of VBD here is that, because it colors vertices, it typically results in much fewer colors as compared to techniques that color constraints/force elements, such as PBD. This is because coloring these elements is equivalent to coloring the nodes of the dual graph, which not only has more nodes, but, more importantly, also has a lot more connections per vertex in general. Examples of this are shown in \autoref{fig:GraphAndColoring}. Since different colors must be handled sequentially, fewer colors means better parallelism.

% \ziheng{Vertex coloring is a method to realize parallelism. Maybe focus more on parallelism. The other parallelism subsection can be renamed as GPU Parallelism or GPU implementation}
%In practice, we do not necessarily need to adjust all the vertices sequentially. We can convert our model to a graph, where each node represents a vertex, and an edge exists iff its two vertices share an element-based energy. Note that this graph is equivalent to the vertex-edge graph of the tetrahedra/triangular mesh (\autoref{fig:GraphAndColoring:a}), but not to the mesh consisting of quad/hexahedron mesh because the diagonal line of a quad/hexahedron is not an edge of the mesh. We can color this mesh, and then the vertices that belong to the same color will not share one element. Therefore, we can parallel the adjustment of those vertices without competing conditions and preserve the property represented by Eq\ref{Eq:VBDStepEnergyChangeProperty}.


%\subsubsection{Collision Handling}

%Now we start to consider collisions. The collision energy can be added to the term $E(\Vec{x})$  as a potential energy to the object energy (\autoref{Eq:VariantionalFormOfImplicitEuler}). A major problem of collision is that it dynamically changes the topology of the model, randomly adding edges to our energy graph. One solution to this is to dynamically redo the coloring based on the collisions, to make sure the collision potential is not shared by vertices within one color. However this coloring procedure can be expensive, and more importantly, has an inconsistent computational cost. This is particularly a problem when collision detection is required for every iteration.

When all force elements are known ahead of the simulation, graph coloring can be performed as a preprocess. However, dynamically generated constraints/force elements, such as ones due to collisions, cannot be known ahead of time, requiring dynamic recoloring.
%Unfortunately, performing dynamic graph coloring can be expensive and can have an unpredictable and substantially varying computation cost, which is particularly a problem for applications with limited computation budgets or when collision detection must be performed after every iteration.

In our implementation for elastic body dynamics, we avoid the cost of recoloring by precomputing coloring only for material forces, ignoring dynamically generated force elements due to collisions.
%Our solution is pre-computing coloring only using the known force elements and entirely skipping re-coloring to consider dynamically-generated force elements due to collisions. 
This means that these collision forces may use multiple vertices of the same color. Therefore, we cannot simply run a parallel loop over all vertices of the same color and update them, because handling a vertex with a dynamically generated force element may run into race conditions (with partially updated vertex positions) when accessing other vertices of the same color.


\del{We resolve this by splitting the processing of a color into two phases, as shown in Algorithm 1. The first phase computes the gradients and Hessians of all force elements acting on vertices of the color without updating any vertex positions. The second phase uses the computed data in the first phase to solve the local system and update the vertex positions. Thus, dynamically generated force elements using multiple vertices of the same color result in (partially) Jacobi-style iterations for those vertices, as opposed to Gauss-Seidel. Everything else follows the Gauss-Seidel order.}

\add{We resolve this by having an auxiliary vertex position buffer ($\vec{x}^{\text{new}}$) that stores the updated vertex position. When executing each local VBD position update, we write the updated vertex positions to the auxiliary buffer, instead of directly overwriting the original vertex position buffer. Then, we copy the updated positions from the auxiliary buffer to the original vertex position buffer after each color pass. This prevents the race conditions that arise from simultaneous read and write operations on vertex positions.

With this process, dynamically generated force elements using multiple vertices of the same color result in (partially) Jacobi-style iterations for those vertices, because they rely on the positions from the previous iteration of those vertices. 
For vertices with different colors, it is equivalent to Gauss-Seidel iterations, considering the updated positions of the vertices with different colors.
Note that our algorithm does not explicitly switch between Jacobi and Gauss-Seidel iterations, but the resulting iteration we describe above corresponds to either (partially) Jacobi or Gauss-seidel, depending on the colors of the colliding vertices.
%this distinction is automatically handled without explicitly separating the approaches in our code. 
%\cem{The meaning is obvious but the sentence is confusing. Removing fixes it.}
}



\begin{figure}
\centering
%\includegraphics[width=\columnwidth]{Figures/08_ExtremeTwist.pdf}
% \includegraphics[width=\linewidth,trim=100 200 150 200, clip]{Figures/BeamRotation/a}\\
\newcommand{\img}[3]{\begin{subfigure}{0.49\linewidth}\centering
\includegraphics[width=\linewidth,trim=#2 100, clip]
{Figures/CollisionResolutionScheme/A00000061-cc}\vspace{-0.5em}
\caption{#3} \label{CollisionResolutionScheme:#1}
\end{subfigure}}
\img{a}{0 0 960}{No recoloring \textbf{(ours)}}\hfill%
\img{b}{960 0 0}{Recoloring}
\caption{Handling collisions using \sref{a}~our scheme without recoloring and \sref{b}~recoloring to achieve perfect Gauss-Seidel iterations, 
%Here the Gauss-Seidel is achieved by naive coloring: giving each colliding vertex a distinct color. 
both simulated using friction forces and accelerated iterations with $\rho=0.95$. Notice that the results are highly similar, though not identical.}
\label{fig:CollisionResolutionScheme}
\end{figure}






One might expect this solution to negatively impact the convergence of VBD. Fortunately, however, such Jacobi-style information exchanges are relatively rare. This is because, as shown in \autoref{fig:CollisionPotential}, with vertex-face collisions at most one pair and with edge-edge collisions at most two pairs of vertices can have the same color. Also, vertices with the same colors must be located on different sides of the collision; therefore, their elastic energies are usually decoupled. This ensures that the majority of the information exchange follows the Gauss-Seidel order and thereby the impact of our solution on convergence is minimal.
\autoref{fig:CollisionResolutionScheme} presents an example with a large number of collisions, comparing our solution of skipping recoloring to proper Gauss-Seidel iterations with recoloring, showing that the differences are minor.
%\cem{It would be good to properly justify this claim by comparing our solution to fully Gauss-Seidel style updates and fully Jacobi style updates for the collision forces: something like \autoref{fig:AccelerationComparison} with (a)~Jacobi, (b)~Ours, and (c)~Gauss-Seidel.}

\del{Another advantage of our two-phase computation is that it results in a workload that is better suited for the GPU. If a single parallel loop is used, for each vertex we must loop over all of its force elements to compute their gradient and Hessian. Since vertices can have different numbers of force elements, this can result in poor occupation with SIMD computation. Our two-phase solution minimizes this and only requires storing 12 numbers (3 for the gradient and 9 for the Hessian of $E_j$) per force element.}

%Note that our solution can also be implemented without the need for the two phases, but instead by storing a copy of vertex positions prior to the update of a color, though the two-phase implementation also helps with better parallelization performance, as we explain below in \autoref{sec:gpu_implementation}.


Our solution also works with other types of topological changes, such as tearing and fracturing. Deleting force elements does not require any changes to vertex coloring. When an object is split by duplicating vertices, as in the case of tearing a piece of cloth along some edges (see \autoref{fig:TopologicalChange}), duplicated vertices can safely inherit the colors of their original vertices.

\add{
\section{GPU Implementation}

% The parallelism of our method allows for a highly-efficient GPU implementation. In this section, we describe the details of our implementation that utilizes both block-level (across multiple warps/wavefronts, i.e. groups of threads) and thread-level (within a warp/wavefront) parallelism.

In this section, we describe a GPU implementation specifically designed to leverage the inherent parallelization mechanism of modern GPUs, which consists of two hierarchical levels: block-level and thread-level parallelism. Block-level parallelism facilitates large-scale parallel operations, assuming that each block operates independently. On the other hand, thread-level parallelism provides finer, single-instruction-multiple-thread (SIMT) style parallelism, allowing for inter-thread communication and synchronization within the same block.

Reflecting on VBD, we observed that it naturally aligns with this hierarchical architecture. We have thousands of vertices within a single color category that operate independently, and each vertex is associated with multiple force elements, which can be processed concurrently.
\autoref{alg:VBDStep} shows the pseudocode of our implementation. It uses block-level parallelism for processing each vertex. The threads within each block are used for computing the forces and Hessians, storing them in local shared memory, and computing the sums via reduction. We use a fixed number of threads for each block.
%, denoted by $n_{t}$.
When the total number of adjacent force elements exceeds the number of threads for each block, individual threads will loop over their assigned elements. During this process, they calculate the forces and Hessians for these force elements and then sum them to their assigned shared memory. 
At last, the forces and Hessians of all the threads are combined using a local reduction sum method (lines 12,13).

% Reflecting on VBD, we observed that it naturally aligns with this hierarchical architecture. We have thousands of vertices within a single color category that operate independently, and each vertex is associated with multiple force elements, which can be processed in parallel. Hence we provide the algorithm described by \autoref{alg:VBDStep}. The cornerstone of this strategy involves assigning a thread block to each vertex  (line 7), as opposed to using a single thread. Within these blocks, each thread concurrently computes the force and Hessian for an adjacent force element, storing the outcomes in the shared memory (lines 8$\sim$11). We allocate a fixed number of threads for each thread block, denoted by $n_{t}$. When the total number of adjacent force elements surpasses $n_{t}$, individual threads are tasked with looping over their assigned elements. During this process, they calculate the forces and Hessians for these elements and then collectively sum these values in their assigned shared memory. At last, the forces and Hessians of all the threads are combined using a local reduction sum method (lines 12,13).

In our experiments, we observed nearly \textit{an order of magnitude performance improvement}, as compared to processing each vertex with a single thread.
%This parallelization mechanism turns out to be remarkably efficient. In our tests, it runs nearly an order of magnitude faster than the trivial parallelization, where a thread is assigned to each vertex to sequentially process its adjacent force elements. 
The primary advantage lies in the optimization of the memory access pattern, a common bottleneck in GPU programs. This implementation reduces memory divergence within blocks.  Because the neighboring force elements of a vertex often share multiple vertices, the threads within the same block can share a  global memory access to those shared vertices. 
Furthermore, this strategy improved the parallelism of the algorithm by allowing parallel evaluation of the force and Hessian of adjacent force elements, which are then written to the significantly faster shared memory. This bypasses the slower global memory and enables the parallel aggregation of force and Hessian values, enhancing the overall efficiency of the process.


% Given that elements adjacent to a vertex create an n-dimensional disc (2 for triangular mesh and 3 for tetrahedral mesh), these neighboring elements often share multiple vertices. For instance, in a tetrahedral mesh, a vertex $\Vec{x}_a$ adjacent to another vertex $\Vec{x}_b$ is shared by at least three, but more commonly over five, neighboring tetrahedra of $\Vec{x}_b$. This shared access can propagate to all threads within the same warp, making a single global memory access far more efficient. Approximately, in our parallelism scheme, one global memory access can be shared by about 5 threads.

%Furthermore, this strategy facilitates parallel processing in evaluating the force and Hessian of adjacent elements, which are then written to the significantly faster shared memory. This bypasses the slower global memory and enables the parallel aggregation of force and Hessian values, enhancing the overall efficiency of the process.
}



\begin{figure}
\centering
\includegraphics[width=0.28\linewidth,trim=250 200 250 150,clip]{Figures/TopologicalChange/a-cc} \hfill%
\includegraphics[width=0.33\linewidth,trim=138 200 148 150,clip]{Figures/TopologicalChange/b-cc} \hfill%
\includegraphics[width=0.35\linewidth,trim=128 200 128 150,clip]{Figures/TopologicalChange/c-cc}
\caption{Tearing a piece of cloth with 2500 vertices and 4800 triangles.}
%Despite running on CPU, this example is taking 11ms/frame.
\label{fig:TopologicalChange}
\end{figure}




\begin{algorithm}[t]
\SetKwFor{Foreach}{for each}{do}{end}
\SetKwFor{DoParallel}{parallel for each}{do}{end}
\newcommand\mycommfont[1]{\footnotesize\textcolor[RGB]{0 128 0}{#1}}
\SetCommentSty{mycommfont}
\LinesNumbered
\DontPrintSemicolon
\SetAlgoNoLine
\KwIn{
$\Vec{x}^t$:  the positions of the previous step;
$\Vec{v}^t$:  the velocities of the previous step;
$\Vec{a}_{\text{ext}}$: the external acceleration
%$[\mathcal{F}_i]$: lists of related collisions for each color
}
\KwOut{This step's position $\Vec{x}^{t+1}$ and velocity $\Vec{v}^{t+1}$.}
$\Vec{y}\gets\Vec{x}^t + h \Vec{v}^t + h^2 \Vec{a}_{\text{ext}}$\;
Initial DCD using $\Vec{x}^t$\;
$\Vec{x}\gets$ initial guess with adaptive initialization\;
\Foreach{\upshape iteration $n\leq n_{\max}$}{
   \lIf{\upshape $n\!\!\mod{n_{\text{col}}}=1$}{CCD using $\Vec{x}$}
   
   \Foreach{\upshape color $c$}{
        
        % \tcp{\del{Phase 1:}}
        % \DoParallel{\upshape force element $j$ in color $c$}{
        %     Compute the gradient and Hessian of $E_j$ wrt. its vertex with color $c$.\;
        % }
        % \tcp{Phase 2:}
        % \DoParallel{\upshape vertex $i$ in color $c$}{
        %     Assemble $\vec{H}_i$ and $\vec{f}_i$ using gradients and Hessians of all force elements acting on vertex $i$.\;
        %     $\Delta \Vec{x}_i \gets \vec{H}_i^{-1} \vec{f}_i$\;
        %     %\uIf{\upshape using line search}{
        %         $\Delta \Vec{x}_i \gets$  optional line search from $\Vec{x}_i + \Delta \Vec{x}_i$ to $\vec{x}_i$\;
        %     %}
        %     $\Vec{x}_i \gets \Vec{x}_i + \Delta \Vec{x}_i$\;
        % }

        \add{
        \tcp{Block-level parallelization} 
        \DoParallel{\upshape vertex $i$ in color $c$}{
            \tcp{Thread-level parallelization }
            \DoParallel{$j\in \mathcal{F}_i$} {
                \tcp{Variables in shared memory}
                $\vec{f}_{i,j} = -\frac{\partial E_j}{\partial  \vec{x}_i}$\; 
                $\vec{H}_{i,j} = \frac{\partial^2 E_j}{\partial \vec{x}_i \partial \vec{x}_i}$\;
            }
            \tcp{Local reduction sums}
            $\vec{f}_i = \sum_{j\in\mathcal{F}_i}\vec{f}_{i,j}$\;
            $\vec{H}_i = \sum_{j\in\mathcal{F}_i}\vec{H}_{i,j}$\;
            
            $\Delta \Vec{x}_i \gets \vec{H}_i^{-1} \vec{f}_i$\;
            %\uIf{\upshape using line search}{
                $\Delta \Vec{x}_i \gets$  optional line search from $\Vec{x}_i + \Delta \Vec{x}_i$ to $\vec{x}_i$\;
            %}
            $\Vec{x}_i^\text{new} \gets \Vec{x}_i + \Delta \Vec{x}_i$\;
        }

        \tcp{Copy updated positions back to the vertex buffer}
        \DoParallel{\upshape vertex $i$ in color $c$}{
            $\vec{x}_i =  \Vec{x}_i^\text{new}$
        }
        }
    }
    
    \tcp{Optional: accelerated iteration}
    \DoParallel{\upshape vertex $i$}{
        Update $\vec{x}_i$ using \autoref{eq:accelerator}.
    }
}        
$\Vec{v} = (\Vec{x} - \Vec{x}^t)/h$\;
return $\Vec{x}$, $\Vec{v}$\;
\caption{VBD simulation for one time step.}
\label{alg:VBDStep}
\end{algorithm}




%To avoid the problem of re-coloring the vertices, we propose a hybrid collision handling scheme. We observe that most collision potentials are defined between either a vertex-face pair or an edge-edge pair, consequently being a function of 4 vertices' positions for tetrahedral meshes, see \autoref{fig:CollisionPotential}. We cannot simply parallelize the VBD solve based on the coloring based on elasticity. If some of those 4 colliding vertices are from one color, there could be competing conditions in accessing their positions because they are getting modified simultaneously. Our hybrid collision handling scheme is designed to avoid this competing condition.
%
%Our solution is to pre-store the collision information used for computing the collision gradient and Hessian and use those stored data when adjusting each vertex to avoid compting conditions. This guarantees there is no competing condition in the computation of the collision. Consequently, the collision handling scheme automatically divides into two methods: Jacobi style for colliding vertices of the same color, and Gauss-Seidel for those of different colors. Leveraging the coloring property, at most one pair of vertices can be resolved via Jacobi style in vertex-face collisions (\autoref{fig:CollisionPotential}a), and a maximum of two pairs in edge-edge collisions (\autoref{fig:CollisionPotential}b). Another observation is that the vertices with the same colors must be located at different sides of the collision, therefore their elastic energies are usually decoupled. This ensures the majority of collisions are addressed through Gauss-Seidel iteration.
%
%It is important to note that this separation occurs naturally due to the utilization of pre-stored collision information, and both collision types are resolved using identical solutions.
%
%The Hybrid Collision handling scheme requires the algorithm to maintain a list of related collisions for each color. We create those lists simultaneously with collision detection using atomic operation.
%
%Other than this hybrid handling method, we also acknowledge that there are alternative solutions to avoid the competing conditions, one example is having 2 vertex position buffers and alternates to read from one and write to the other. This particular scheme is better suited for scenarios with less intensive collisions as it does not require a distinct collision sweep.



%\subsubsection{Topological Changes} Our simulation operates without relying on a global system, allowing for flexible handling of topological changes. Here we demonstrate an example of tearing cloth. The cloth tears along the edges, therefore no new triangle is created during the tearing. To tear each edge, we duplicate a vertex, modify the vertex list of the affected triangles, and adjust the adjacent triangle list for the duplicated vertices. This method proves highly efficient. Additionally, the duplicated vertices can directly inherit the color of the original vertex.



\begin{comment}

\section{Implementation Details}
\label{sec:gpu_implementation}

VBD's strength lies in its exceptional parallelism, allowing a better utilization of GPU computation. In this section, we provide some important details of our GPU implementation.
%enabling it to harness the full potential of GPU processing. In this context, we're introducing customized parallelization techniques tailored for GPU utilization, aiming to enhance and fully leverage this inherent parallelism in VBD.

%\subsection{Hybrid Sweeps}

The most time-consuming part of our method is the evaluation of the gradient and Hessian. Since each vertex has a varying number of force elements acting on it, a straightforward parallelization by vertex would result in for-loops of different lengths, thereby reducing GPU core occupation.
%, introducing branching in the kernel and causing a slowdown in computation.
Fortunately, our two-phase solution described in \autoref{sec:parallelism} addresses this. We simply
%To address this, we aim to minimize unsynchronized computations by leveraging a distinctive property of VBD. We can gather all tetrahedra adjacent to 
keep a list of all force elements using
vertices of a specific color and loop over this list in parallel to compute the gradient and Hessian for all force elements in the first phase. 
%vertices with that color. 
Notably, vertices with the same color do not share force elements, except for dynamically-created ones, which can be duplicated in this list for each vertex of the same color.
For each force element $j$ in this list, we only require storing 12 floating-point numbers: 3 for the gradient and 9 for the Hessian of its energy $E_j(\vec{x})$.
%, therefore each tet requires only 12 floating-point numbers for storage: 3 for gradient ($\frac{\partial E_t}{\partial \Vec{x}_k}$) and 9 for the Hessian ($\frac{\partial ^ 2 E_t}{\partial \Vec{x}_k \partial \Vec{x}_k}$). This process can be parallelized by tetrahedra, termed "tet sweep".

%Similarly, we conduct a collision sweep, grouping collisions associated with vertices of the same color for parallel processing. Within each collision sweep, we update collision information and precompute the intermediate results of the collision gradient and Hessian evaluation. The final stage involves a vertex sweep that sums up the gradients and Hessians evaluated from the previous step, solves the linear system, and optionally, does a local line search.

%We've observed that this three-stage hybrid sweep can enhance our GPU implementation by up to 20\%. However, we've also noted that it doesn't notably accelerate our CPU implementation. The GPU-based version of our approach is detailed in Algorithm Alg.\ref{alg:VBDStep}.

The second phase is the parallel computation of all local systems for all vertices of the same color. This uses the force element gradients and Hessians computed in the first phase. \autoref{alg:VBDStep} shows the pseudocode of our implementation.



\begin{algorithm}[t]
\LinesNumbered
\SetAlgoNoLine
\KwIn{
$\Vec{x}^t$:  the positions of the previous step;
$\Vec{v}^t$:  the velocities of the previous step;
$\Vec{f}_{ext}$: the external force;
$[\mathcal{C}_i]$: lists of related collisions for each color
}
\KwOut{This step's position $\Vec{x}^{t+1}$ and velocity $\Vec{v}^{t+1}$.}
$\Vec{y}=\Vec{x}^t + h \Vec{v}^t + h^2 \Vec{f}_{ext}$\;
initial discrete collision detection using $\Vec{x}^t$ \;
$\Vec{x}=getInitialGuess()$\;
\For{$j$ in $N_{\text{iteration}}$}{
   \SetKwBlock{DoParallel}{parallel for}{end}
    collision detection using $\Vec{x}$ \;
   
   \For{$i$ in colors}{
        \DoParallel ($t$ in tets adjacent to vertices in color){
            compute $E_t$'s gradient and hessian wrt. its vertex with color $i$\;
        }

        \DoParallel ($c$ in $\mathcal{C}_i$){
            update and precompute information for $c$\;
        }

        \DoParallel (vertex $k$ in color $i$){
            assemble the Hessian $H_k$ and gradient $\frac{\partial g_k}{\partial x_k}$ \;
            % compute force $\Vec{f}_k = -\frac{\partial g_k}{\partial x_k} + \Vec{f}_{ext}$ \;
            $\Delta \Vec{x}_k = -H_k ^ {-1} \frac{\partial g_k}{\partial x_k}$\;
            \uIf{do line search}{
                $\Delta \Vec{x}_k =  backTracingLineSearch(\Vec{x}_k, \Delta \Vec{x}_k)$\;
            }
            $\Vec{x}_k \gets \Vec{x}_k + \Delta \Vec{x}_k$\;
        }
    }
}        
$\Vec{v} = (\Vec{x} - \Vec{x}^t$)/h\;
return $\Vec{x}$, $\Vec{v}$\;
\caption{VBD Simulation Step on GPU \cem{OLD}}
\label{alg:VBDStepOLD}
\end{algorithm}


%\subsection{Computational Load Equilibrium}

In our tests with deformable objects, our vertex coloring typically produces less than 10 colors for tetrahedral meshes and less than 5 colors for triangular meshes.
%As we have discussed vertex coloring usually generates less than 10 colors for tet meshes and less than 5 for triangular meshes. 
Having such a small number of colors (as opposed to coloring based on constraints/force elements) is ideal for parallelism. However, unless a balanced coloring algorithm is used (e.g. \cite{Giannoula2023}), some colors may not include a large number of vertices to fully utilize all GPU cores.
%However, the coloring usually presents a problem: the uneven distribution of vertices among colors leads to a significant imbalance of computational load. 
%To address this, we propose a simple scheme for scenarios involving multiple models, which is based on combining the smaller-sized color of one model with the larger-sized color of another. 
For simulations involving multiple objects, we address this by combining the colors of different objects, such that we form a balanced stack of colors for the whole system.
%Let's say we have $L$ models that we aim to solve collectively, requiring a number of colors equivalent to the maximum color count of each model. Initially, every color begins empty. Our approach involves merging colors from these models into combined colors using a best-fit strategy: always add it to an available color with the smallest size. After one color of the mesh is added to a combined color, the other colors of this mesh cannot be added to this combined color again.
We achieve this using a simple greedy algorithm that allocates as many global colors as the maximum number of colors for all objects. Then, for each object, its colors, in descending order of size, are combined with the global color of the smallest size \anka{This is not precise; after adding one color to the smallest global color, the global color can still be the smallest. However, you cannot add the next object color to this global color.}. While this simple approach does not guarantee an optimal balance, it can avoid having global colors with too few vertices in practice, as shown in \autoref{fig:LoadEquilibrium}.

\end{comment}



==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/04_Results.tex <==
\begin{figure*}
\centering
%\includegraphics[width=\columnwidth]{Figures/12_SovlingExistingCollision_Spaghetti.pdf}
\newcommand{\fig}[1]{\fbox{\includegraphics[width=0.245\linewidth,trim=350 0 450 0,clip]{Figures/SquishyBallsToTeapot/#1-cc}}}
\fig{A00000130}\hfill%
\fig{A00000370}\hfill%
%\fig{A00000610}\hfill%
\fig{A00001030}\hfill%
\fig{A00001510}
%\caption{Our method can start with a \textit{(a)} initial state with extremely deep self-intersections and revert from deep self-intersections \textit{(b,c)} back to a state \textit{(d)} where all the collisions are properly handled. }
\caption{Simulation of 216 squishy balls with tentacles, a total of 48 million vertices and 151 million tetrahedra, dropped into a Utah teapot, forming a stable pile with active frictional contacts. The average and maximum computation time per time step is \del{10 and 16} \add{3.6 and 3.9} seconds, respectively, using $S=4$ substeps per frame and $n_{\max}=40$ iterations per step. The final frame of this simulation is shown in \autoref{fig:teaser}.}
\label{fig:SquishyBallsToTeapot}
\end{figure*}

\begin{figure*}
\centering
%\includegraphics[width=\columnwidth]{Figures/12_SovlingExistingCollision_Spaghetti.pdf}
\newcommand{\fig}[1]{\fbox{\includegraphics[width=0.245\linewidth,trim=250 0 250 0,clip]{Figures/HybrridModelsDropping/#1-cc}}}
\fig{a}\hfill%
\fig{b}\hfill%
\fig{c}\hfill%
\fig{d}\vspace{-0.043\linewidth}\\
%\hfill\fig{e}
%\newcommand{\scap}[2]{\begin{minipage}{#2\linewidth}~\small\textbf{(#1)}\end{minipage}}
%\vspace{-1.6em}
%\scap{a}{0.2}%
%\scap{b}{0.2}%
%\scap{c}{0.2}%
%\scap{d}{0.2}%
%\scap{e}{0.2}\vspace{0.2em}
%\caption{Our method can start with a \textit{(a)} initial state with extremely deep self-intersections and revert from deep self-intersections \textit{(b,c)} back to a state \textit{(d)} where all the collisions are properly handled. }
\hspace*{0.5\linewidth}%
\begin{minipage}{0.25\linewidth}\centering
\scriptsize\color{white} $\uparrow$ This platform\\will be removed.
\end{minipage}%
\hspace*{0.5\linewidth}\vspace{0.8em}
\caption{Simulation of 10,368 deformable objects, totaling over 36 million vertices and 124 million tetrahedra, dropped onto a platform inside a box container. Then, the platform is suddenly removed and the objects collectively fall onto the ground, forming stable piles both before and after the platform is removed.
The average and maximum computation times per time step are \del{12 and 14} \add{4.2 and 4.7} seconds, respectively, using $S=2$ substeps and $n_{\max}=60$ iterations per step. 
%\anka{In this and the next figure you use computational time per step but in the text you use time per frame.}\cem{Intentional. Otherwise, I will need to explain substeps per frame, which is too much unnecessary detail for the text.}
The final frame of this simulation is shown in \autoref{fig:teaser}.}
\label{fig:HybrridModelsDropping}
\end{figure*}



\section{Results}

We evaluate our method with elastic body dynamics qualitatively with various tests and quantitatively with \del{direct} comparisons to alternative methods.
%
We use Neo-Hookean \cite{smith2018stable} materials (without the logarithmic term) for our volumetric objects, StVK \cite{Volino09} for clothes, and linear springs for elastic rods.

We use a fixed frame time of $1/60$ seconds and a fixed iteration count $n_{\max}$, instead of estimating convergence after every iteration. Each frame is computed using $S$ substeps, such that ${h=1/(60S)}$ seconds. Using smaller time steps increases accuracy and reduces numerical damping with any implicit Euler method. With VBD, a smaller time step only requires fewer iterations per step for similar visual quality, but it can also achieve a smaller residual with the same number of total iterations per frame (i.e., $S n_{\max}$).
\add{The number of threads per block is set to 16 for all the experiments.}

We use no line search in our tests, as none of our tests required it for stability, and running line search can result in a noticeable drop in performance. 
% Unless noted, our results do not include accelerated iterations. 
In our experiments, we apply CCD only in the first iteration (i.e. $n_{\text{col}}=n_{\max}$), unless otherwise specified.

In our implementation, we handle collisions on the CPU using Intel's Embree library \cite{wald2014embree}. The two phases with parallel loops are implemented on the GPU using CUDA.
%
All timing results are generated on a computer with an AMD Ryzen 5950X CPU, 64GB DDR3 RAM, and an NVIDIA RTX 4090 GPU.
The runtime statistics and parameters of all our experiments can be found in \autoref{Table:statistics}.
%, and 64GB of DDR3 3200MHz RAM.

%We generate our results on a computer with an AMD Ryzen 5950X CPU, an NVIDIA RTX 4090 GPU, and 64GB of DDR3 3200MHz RAM. Our collision detection is implemented using Intel's Embree library \cite{wald2014embree}. All other parts are implemented on GPU using CUDA. We use NeoHookean material for our volumetric simulation, and StVK for the clothes simulation. 
%We also implemented the preconditioned gradient descent method \cite{wang_descent_2016} and Newton's method for comparison. The gradient descent method is also implemented using CUDA. For Newton's method, we use the direct Cholesky (LDLT) factorization solver provided by Intel's MKL library \cite{wang2014intel}. 
%Despite the difference in the simulation time step, the frame time is evaluated based on the computational time of 1/60s of the simulation.



\subsection{Large-Scale Tests}

In \autoref{fig:teaser} we present two large-scale test, showcasing our method's performance, scalability, and stability in scenarios involving a large number of complex collisions, including stacking and rest in contact.

The first one has 216 squishy balls with tentacles, totaling 48 million vertices and 151 million tetrahedra acting as force elements, dropped into a Utah teapot. Intermediate frames of this simulation are shown in \autoref{fig:SquishyBallsToTeapot}.

The second one includes more than 10 thousand deformable objects, 
%\anka{why not say the exact number: 10368}\cem{because the exact count is not important and "10 thousand" is easier to read.}
totaling over 36 million vertices and 124 million tetrahedra, dropped into a box and piled on a platform, which is then suddenly removed, making the pile collectively fall onto the ground. The intermediate frames are shown in \autoref{fig:HybrridModelsDropping}.

As can be seen in our supplemental video, both of these simulations exhibit stable motion, quickly forming static piles, while maintaining rest-in-contact behavior with over 1 million active collisions.
VBD's parallelism and fast convergence resulted in an average computation time of 40 and 25 seconds per frame in these simulations, respectively.

%Due to VBD's excellent parallelism and fast convergence, we are capable of simulating extensive scenes involving complex collisions within a reasonable computational timeframe. \autoref{fig:SquishyBallsToTeapot} showing 216 squishy balls dropping into a rigid teapot container. Additionally, we showcase the release of 10,368 mixed models, including bunnies, armadillos, teapots, and octopi, into a two-layered container as depicted in \autoref{fig:HybrridModelsDropping}. Once all models have descended, we proceed by removing the container's middle layer, allowing all components to drop simultaneously (\autoref{fig:HybrridModelsDropping}de). Remarkably, both experiments resulted in the formation of stable piles, maintaining rest-in-contact with over 1 million active collisions. These experiments encompassed managing over 100 million Degrees of Freedom (DoFs), a scale surpassing any prior single GPU simulation by at least an order of magnitude, to the best of our knowledge. 






\begin{figure}
\centering
%\includegraphics[width=\columnwidth]{Figures/08_ExtremeTwist.pdf}
% \includegraphics[width=\linewidth,trim=100 200 150 200, clip]{Figures/BeamRotation/a}\\
\fbox{\includegraphics[width=\linewidth,trim=180 0 120 20, clip]{Figures/ElasticityConvergence/bending-cc}}
\caption{Visual convergence with different numbers of iterations per frame for different material stiffness (with accelerated iterations using ${\rho=0.75,0.86,0.93}$ top to bottom), simulating a beam with 463 vertices and 1.5 thousand tetrahedra.
%Showcasing the convergence property of method. We simulate a beam (463 vertices and 1.5K tetrahedra) sagging under gravity with one end fixed using a time step of 1/300s. By adjusting stiffness and varying the number of iterations, we generate a 3$\times$3 grid of simulations, along with the reference results generated by the converged Newton's method.
}
\label{fig:ElasticityConvergence}
\end{figure}

\subsection{Unit Tests}

%\subsubsection{Elasticity}
The convergence rate of VBD depends on the stiffness of the simulated system. This is demonstrated in \autoref{fig:ElasticityConvergence}, comparing VBD with different numbers of iterations per frame to the converged solution computed using Newton's method.
%In \autoref{fig:ElasticityConvergence} we showcase our method's convergence behavior across different stiffness. For each stiffness, we also provide a reference result given by running Newton's method until it converges. 
As expected, VBD converges slower for stiffer materials, which is common for descent-based solvers. In this example, 15 iterations are more than sufficient for the softest material, while stiffer ones require more. 
As can be seen in our supplemental video, even though VBD can qualitatively imitate the behavior of stiff materials with a relatively small number of iterations, the motion can quickly diverge from the converged solution, due to the remaining residual, unless a sufficient number of iterations are used.
%While VBD can achieve highly stiff behavior with 5 for moderately stiff materials, and only 10 for the stiffest material. Please see our supplementary video for the dynamic sequence.




\begin{figure}
\centering
%\includegraphics[width=\columnwidth]{Figures/08_ExtremeTwist.pdf}
% \includegraphics[width=\linewidth,trim=100 200 150 200, clip]{Figures/BeamRotation/a}\\
\newcommand{\acap}[3]{\begin{minipage}{#1\linewidth}~\vspace{#2em}\\#3\end{minipage}}
\includegraphics[width=\linewidth,trim=0 0 150 200, clip]{Figures/FrictionUnitTest/aa-cc}\vspace{-0.52\linewidth}\\
\hfill%
\acap{0.17}{0.0}{$\mu_c=0.0$}%
\acap{0.17}{0.2}{$\mu_c=0.3$}%
\acap{0.20}{0.4}{$\mu_c=0.6$}%
\acap{0.16}{0.8}{$\mu_c=0.9$}\vspace{0.44\linewidth}\\
\newcommand{\scap}[2]{\begin{minipage}{#2\linewidth}\centering{$\mu_c=#1$}\end{minipage}}
\newcommand{\figT}[1]{\includegraphics[width=0.25\linewidth,trim=580 0 680 260, clip]{Figures/FrictionUnitTest/#1-cc}}
\figT{0.0}\hfill%
\figT{0.2}\hfill%
\figT{0.4}\hfill%
\figT{0.6}\vspace{-7.8em}
\scap{0.0}{0.25}%
\scap{0.2}{0.25}%
\scap{0.4}{0.25}%
\scap{0.6}{0.25}\vspace{6.4em}
\caption{Testing different friction coefficients $\mu_c$ for \sref{top}~an elastic cube with 400 vertices and 1.45 thousand tetrahedra, initially resting on an incline, and \sref{bottom}~4 elastic octopus models, totaling 15.6 thousand vertices and 60 thousand tetrahedra, dropped into a box.
%Visualizing the impact of diverse friction ratios through two scenarios. The upper section depicts cubes sliding down $30^{\circ}$ slopes, each showcasing distinct friction ratios. The lower section demonstrates the behavior of thrown 4 octopuses with varied friction ratios, forming piles varying in height and structure. Simulated using friction forces.
}
\label{fig:FrictionUnitTest}
\end{figure}

%\subsubsection{Friction and Damping}
We present our tests with different friction coefficients $\mu_c$ for friction forces in \autoref{fig:FrictionUnitTest}. Notice that, $\mu_c$ impacts the motion, as expected, and with sufficiently high $\mu_c$, we can properly preserve the position on an incline and form taller piles.
%\autoref{fig:FrictionUnitTest}. The upper section visualizes cubes sliding down $30^{\circ}$ slopes with different friction ratios, demonstrating our capability to manage the transition between dynamic and static frictions. The lower section showcases stacking the models with different friction ratios. Upon being dropped into a box, these models form piles exhibiting varying heights and distinct structures.


In our supplemental video, we also include a comparison of different damping stiffness $k_d$, showing that, despite numerical damping of implicit Euler, without damping we can preserve kinetic energy for a long time. As we increase $k_d$, the motion subsides quicker, as expected.
%visualization showcasing the impact of various damping parameters. Please see our supplementary video.



\subsection{Stress Tests}

We present a challenging frictional contact case in \autoref{fig:ExtremeTwist}, twisting two thin beams together. This example includes extreme deformations, generating strong material forces that compete with self-collisions and collisions between the two beams. It is simulated with collision detection occurring 
%with CCD \anka{not CCD! DCD} 
once every 5 iterations (i.e. $n_{\text{col}}=5$). Notice that VBD can properly handle such strong deformations with frictional contact.
%In \autoref{fig:ExtremeTwist} we show twisting two thin beams where noticeable buckling appears. This example showcases extreme deformation, effectively illustrating the complexities of frictional contacts amidst substantial internal forces.

We show two simulations in \autoref{fig:ExtremeInitialization} for stress-testing the stability of VBD under extreme deformations. The first one shows an armadillo model that is perfectly flattened and the second one is a Utah teapot model with all vertices randomly scrambled and placed on the surface of a sphere. Even though the simulations begin with these extremely unstable energy configurations, VBD quickly recovers these models without performing a line search and using 100 iterations per frame.

%We showcase the stability of our method in handling extreme deformations in \autoref{fig:ExtremeInitialization}. This is exemplified through initializing a model, either by flattening it or by randomly projecting its vertices onto a sphere. Despite these challenging conditions, we still use a fixed step size of 1.0 without employing a line search. After the simulation started, both model were able to quickly recover to their original shape.




\begin{figure}
\centering
\newcommand{\img}[3][500 250 600 200]{\begin{subfigure}{0.327\linewidth}%\flushright
\fbox{\includegraphics[width=\linewidth,trim=#1,clip]{Figures/ExtremeStretch/A0000#2-cc}}\vspace{-1.4em}\\
%\label{fig:ExtremeStretch:#3}
%\caption{}
\small\hspace*{0.2em}\textbf{(#3)}\hspace*{0.2em}
\end{subfigure}}
\img{0120}{a}\hfill%
\img{0704}{b}\hfill%
\img{0725}{c}\vspace{0.2em}\\
\img{0738}{d}\hfill%
\img[500 325 600 125]{0757}{e}\hfill%
\img[500 400 600 50]{1319}{f}\\
\caption{A stress test with extreme stretching: a Stanford bunny model with 1.8 thousand vertices and 5.9 thousand tetrahedra is stretched by slowly pulling 10 vertices away, which are then suddenly released. The model recovers its shape after going through considerable deformations and high-velocity motion, simulated with self-collisions and using $S=5$ substeps and $n_{\max}=10$ iterations per step.}
\label{fig:ExtremeStretch}
\end{figure}


Another stress test is shown in \autoref{fig:ExtremeStretch}. In this case, 10 vertices of a Stanford bunny model are first slowly pulled away, generating a state with considerable potential energy, and then suddenly released (right after \autoref{fig:ExtremeStretch}b), causing severe deformations. Once again, VBD successfully handles this challenging simulation case, involving self-collisions with high-velocity impacts, using only $n_{\max}=10$ iterations per step and $S=5$  per frame.
\begin{figure}
\centering
\newcommand{\img}[1]{\begin{subfigure}{0.33\linewidth}\centering
\fbox{\includegraphics[width=\linewidth,trim=420 220 800 100,clip]{Figures/StabilityUnderResidual/A00000#1-cc}}
\end{subfigure}}
\img{100}\hfill%
\img{300}\hfill%
\img{500}
\caption{A stress test using only a single iteration per frame (i.e. a time step of $h=1/60$ seconds and $n_{\max}=1$). One vertex on the armadillo model's nose is pulled while the finger and toe vertices are fixed. The model has 15 thousand vertices and 50 thousand tetrahedra.}
\label{fig:ExtremeStretch2}
\end{figure}
\autoref{fig:ExtremeStretch2} presents a stability test under large residuals by using only a single iteration per frame (i.e. $S=1$ and $n_{\max}=1$). Notice that our method produces stable deformations with extreme stretching, even though the simulation lacks a sufficient iteration count to properly reduce the residual at each frame.



\begin{figure*}
\centering
%\newcommand{\cmpA}[1]{%
%\belowbaseline[0.005\linewidth]{\fbox{\includegraphics[width=0.175\linewidth,trim=780 140 470 50,clip]{Figures/ConvergenceComparisonQuantative/Rendered#1-cc}}}\hfill%
%\belowbaseline[0pt]{\includegraphics[width=0.4\linewidth]{Figures/ConvergenceComparisonQuantative/energyByIter_armadillo#1}}%
%\belowbaseline[0pt]{\includegraphics[width=0.4\linewidth]{Figures/ConvergenceComparisonQuantative/energyByTime_armadillo#1}}}
%\cmpA{}\\
%\cmpA{_stiffer}
\newcommand{\cmpB}[1]{%
\belowbaseline[0.005\linewidth]{\fbox{\includegraphics[width=0.22\linewidth]{Figures/ConvergenceComparisonQuantative/combined_#1-cca}}}\hfill%
\belowbaseline[0pt]{\includegraphics[height=0.255\linewidth]{Figures/ConvergenceComparisonQuantative/energyByIter_armadillo2_#1}}%
\belowbaseline[0pt]{\includegraphics[height=0.255\linewidth]{Figures/ConvergenceComparisonQuantative/energyByTime_armadillo2_#1}}}
\cmpB{soft}
\cmpB{stiff}
\caption{Convergence of different descent methods for simulating an armadillo model with 15 thousand vertices and 50 thousand tetrahedra with \sref{top} a relatively soft material and \sref{bottom} a 10$\times$ stiffer material. Vertices near the top inside the glass block are fixed and the models are initially stretched, as shown on the left, by pulling down foot vertices. Then, the position constraints on foot vertices are suddenly removed, allowing the model to deform for 33 ms. The deformation is computed using a single time step of $h=33$ ms.
%
The graphs show relative loss over iterations and computation time. All methods are implemented on the GPU using the same framework with single precision (32-bit) floating-point numbers, except for Newton's method with Cholesky factorization, which runs on the CPU using double precision (64-bit).
%
Accelerated versions use $\rho=0.95$.}
\label{fig:ConvergenceComparisons}
\end{figure*}

\subsection{Convergence Rate}
To evaluate the convergence rate of VBD, we present a simple test shown in \autoref{fig:ConvergenceComparisons}, where an armadillo model that was previously stretched is suddenly released. Here, we calculate the relative loss after each iteration and compare it to alternative solvers.

The first alternative is preconditioned gradient descent (GD) \cite{wang_descent_2016} implemented on GPU within the same framework as ours. GD requires a form of line search for stability, which is implemented as testing the variational energy after every 8 iterations and, when needed, reducing the optimization step size and backtracking (following the implementation of \citet{wang_descent_2016}). We also include a version of GD that is accelerated using the Chebyshev semi-iterative approach \cite{wang_chebyshev_2015}, as our method. 
The iterations of GD are about \del{3$\times$}\add{30\%} faster than ours \add{without line search. However, it necessitates line search for stability. This makes it about 10\% slower than our VBD, which does not need line search.} \del{but}\add{Furthermore,} its 
convergence rate per iteration is considerably slower, as it corresponds to Jacobi iterations. In this example, when combined with acceleration, GD \del{outperforms}\add{performs similar to} our method without acceleration but lags significantly behind our method with acceleration.

We also compare to a version of our method that uses Jacobi iterations, called \emph{Block Jacobi}, implemented by computing the position change for all vertices in parallel and then applying the position update simultaneously to all vertices at the end of each iteration. We incorporate the same line search scheme as GD for Block Jacobi\add{, as it is necessary for stability}. Block Jacobi outperforms GD, as it uses vertex blocks for computation, which corresponds to using a diagonal Hessian block as a precondition, as opposed to just a diagonal line that GD uses. \del{It also}\add{Without line search, it} achieves \add{20\%} faster iteration times than \del{ours}\add{our VBD}, due to its perfect vertex-level parallelization (without any coloring). However, \add{combined with line search, its iterations are about 17\% slower than VBD. More importantly,} because it uses Jacobi iterations, its convergence is hindered, as compared to our Gauss-Seidel iterations.

Furthermore, we compare \del{our method's}\add{the} convergence \add{of our method} to \add{two implementations of} Newton's method\add{: first} using a direct Cholesky (LDLT) factorization solver provided by Intel's MKL library \cite{wang2014intel} \add{running on the CPU, and the second using a GPU-based conjugate gradient (CG) method.}
To ensure convergence, we do a PSD projection for each tet's Hessian of elasticity. Newton's method uses a line search for each iteration. Since its iterations are slow, the computational overhead of line search is negligible. Though the convergence of Newton's method per iteration is far superior to all others, because of its expensive computation time per iteration, in these examples it lags far behind. Nonetheless, for relatively tame experiments with less stretching and motion, and especially for highly stiff and high-resolution simulations that are much more expensive to simulate, we would expect Newton's method to eventually overtake all alternatives beyond a certain level of convergence.

\add{Finally, we compare our method to a quasi-Newton approach using Laplacian preconditioning \cite{liu_quasi-newton_2017}. We utilize a GPU-based conjugate gradient solver, similar to the one employed in our GPU-CG Newton's method's implementation. Laplacian preconditioning accelerates each linear solve, as it eliminates the need for PSD projection and involves solving a smaller system. Practically, this method demonstrates faster convergence than Newton's method, particularly in the initial stages of the optimization process. Nevertheless, it still lags behind both the accelerated and non-accelerated versions of our VBD.}
\begin{figure}
\centering
\includegraphics[width=0.85\linewidth]{Figures/ConvergenceComparisonQuantative/energyByTime_armadillo2_singleThreaded_stiff.pdf}
\caption{\add{Comparing a single-threaded CPU implementation of our method with single-threaded Newton’s method (using both CG and Cholesky). The scene is identical to the bottom row of \autoref{fig:ConvergenceComparisons} .}}
\label{fig:singleThreaded}
\end{figure}
\add{A part of the performance advantages of our VBD method presented above is related to its efficiency in parallel execution on the GPU. To demonstrate its convergence in the absence of parallel computation, we include a comparison using single-threaded CPU implementations of our VBD and Newton's method with Cholesky factorization and CG. \autoref{fig:singleThreaded} shows the convergence results for the same experiment in the bottom row of \autoref{fig:ConvergenceComparisons}.
In these tests, 
%We conducted an ablation experiment to compare a single-threaded CPU implementation of our method with single-threaded implementation of Newton's method using both CG and Cholesky solvers. This experiment evaluates each method's efficiency to reduce error within a fixed computational budget, independently of parallelism. The results are illustrated in \autoref{fig:singleThreaded}. Initially, 
our method initially demonstrates faster convergence than both versions of Newton's method. Over time, the CG-based Newton's method catches up to our VBD without Chebyshev acceleration. However, VBD with Chebyshev acceleration maintains a significant performance lead over the others. This experiment shows that the performance advantages of our method are not only due to its GPU parallelism.}
%, but also due to a better convergence/computation ratio.


\begin{table*}[]
\caption{Performance results and simulation parameters.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l||lll|lll|ll|ll|l|}
\hline
Experiment Name                & \multicolumn{3}{l|}{Number of}                                  & \multicolumn{3}{l|}{Material}                                                             & \multicolumn{2}{l|}{Contact \&Friction}           & \multicolumn{2}{l|}{Simulation Parameters}  & Time per step                     \\
                               & \multicolumn{1}{l|}{Vert.} & \multicolumn{1}{l|}{Tet.}  & Color & \multicolumn{1}{l|}{Type}       & \multicolumn{1}{l|}{Stiffness}                & Damping & \multicolumn{1}{l|}{$k_c$} & $\mu_c, \epsilon_v$ & \multicolumn{1}{l|}{$h$(sec.)} & Iterations & avg./max                           \\ \hline
Twisting Thin Beams (\autoref{fig:ExtremeTwist})           & \multicolumn{1}{l|}{97K}   & \multicolumn{1}{l|}{266K} & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu = 5e4, \lambda=1e6$} & 1e-6    & \multicolumn{1}{l|}{1e6}   & 0.1, 1e-2           & \multicolumn{1}{l|}{1/300}     & 100        & \del{120/156ms} \add{60/78ms}\\

Flattening initialization  (\autoref{fig:ExtremeInitialization})    & \multicolumn{1}{l|}{15K}   & \multicolumn{1}{l|}{50K}   & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=2e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{NA}    & NA                  & \multicolumn{1}{l|}{1/60}      & 100        & \del{6.6/7.6ms}
\add{3.3/3.8ms}\\

Random initialization  (\autoref{fig:ExtremeInitialization}) & \multicolumn{1}{l|}{2K}    & \multicolumn{1}{l|}{8.5K}  & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=2e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{NA}    & NA                  & \multicolumn{1}{l|}{1/60}      & 100        & \del{5.1/5.6ms}
\add{2.6/2.8ms}\\



Tetmesh Pendulum  (\autoref{fig:AdaptiveInitialization}) & \multicolumn{1}{l|}{304}   & \multicolumn{1}{l|}{755}   & 6     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=1e7,  \lambda=1e8$}  & 0       & \multicolumn{1}{l|}{NA}    & NA                  & \multicolumn{1}{l|}{1/300}     & 20         & <0.1ms \\


Squishy Ball Drops (Figure.\ref{fig:AccelerationComparison},\ref{fig:CollisionResolutionScheme},\ref{fig:CompareToXPBD_TimeStep}) & \multicolumn{1}{l|}{230K}  & \multicolumn{1}{l|}{700K}  & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=2e6,  \lambda=2e7$}  & 1e-7    & \multicolumn{1}{l|}{1e7}   & 0.1, 1e-2           & \multicolumn{1}{l|}{1/120}     & 120        & \del{30/34ms}
\add{15/17ms}\\


Tearing Cloth (\autoref{fig:TopologicalChange}) & \multicolumn{1}{l|}{2500}  & \multicolumn{1}{l|}{4800}  & 3     & \multicolumn{1}{l|}{StVK}       & \multicolumn{1}{l|}{$\mu=1e4,  \lambda=1e4$}  & 1e-5    & \multicolumn{1}{l|}{NA}    & NA                  & \multicolumn{1}{l|}{1/300}     & 20         & 11.2/11.5 ms(cpu)                 \\

Dropping 216 Squshy Balls (\autoref{fig:SquishyBallsToTeapot}) & \multicolumn{1}{l|}{48M}   & \multicolumn{1}{l|}{151M}  & 9     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=2e6,  \lambda=2e7$}  & 1e-7    & \multicolumn{1}{l|}{1e7}   & 0.1, 1e-2           & \multicolumn{1}{l|}{1/240}     & 40         & \del{5.3/7.9s}
\add{3.6/3.9s}\\

Dropping 10368 Models (\autoref{fig:HybrridModelsDropping}) & \multicolumn{1}{l|}{36M}   & \multicolumn{1}{l|}{124M}  & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=1e6,  \lambda=1e7$}  & 1e-7    & \multicolumn{1}{l|}{1e7}   & 0.1, 1e-2           & \multicolumn{1}{l|}{1/120}     & 60         & \del{6.3/7.7s}
\add{4.2/4.7s}\\

Beam Sagging  (\autoref{fig:ElasticityConvergence}) & \multicolumn{1}{l|}{463}   & \multicolumn{1}{l|}{1.5K}  & 6     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=1e6/3e6/1e7$}  & 1e-6    & \multicolumn{1}{l|}{NA}   & NA& \multicolumn{1}{l|}{1/300}     & 3/5/10         & avg.: \del{0.15/0.30/0.54ms}
\add{0.08/0.12/0.24ms}\\

 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{}  &      & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\lambda=1e7/3e7/1e8$}  &    & \multicolumn{1}{l|}{}   & NA& \multicolumn{1}{l|}{}     &         & max: \del{0.16/0.32/0.63ms}
\add{0.08/0.16/0.31ms}\\


Cude Sliding  (\autoref{fig:FrictionUnitTest}) & \multicolumn{1}{l|}{800}   & \multicolumn{1}{l|}{2.9K}  & 6     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=1e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{1e7}   & 0/0.3/0.6/0.9, 1e-2 & \multicolumn{1}{l|}{1/300}     & 10         & \del{0.20/0.31ms}
\add{0.10/0.17ms}\\

Octopi Stacking (\autoref{fig:FrictionUnitTest}) & \multicolumn{1}{l|}{15.6K} & \multicolumn{1}{l|}{60K}   & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=1e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{1e7}   & 0/0.1/0.4/0.6, 1e-2 & \multicolumn{1}{l|}{1/300}     & 10         & \del{1.6/2.0ms}
\add{1.1/1.3ms}\\

% Extreme Stretch with 1 iter.  (\autoref{fig:ExtremeStretch}) & \multicolumn{1}{l|}{1.8K}  & \multicolumn{1}{l|}{5.9K}  & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=2e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{1e7}   & 0.2, 1e-2           & \multicolumn{1}{l|}{1/300}     & 10         & 1.6/2.0ms                         \\

Extreme Stretch  (\autoref{fig:ExtremeStretch2}) & \multicolumn{1}{l|}{1.8K}  & \multicolumn{1}{l|}{5.9K}  & 8     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=2e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{1e7}   & 0.2, 1e-2           & \multicolumn{1}{l|}{1/300}     & 10         & \del{0.86/1.02ms}
\add{0.36/1.02ms}\\

2 Cube colliding (\autoref{fig:CompareToXPBD_MassRatio}) & \multicolumn{1}{l|}{800}   & \multicolumn{1}{l|}{2.9K}  & 6     & \multicolumn{1}{l|}{NeoHookean} & \multicolumn{1}{l|}{$\mu=1e6,  \lambda=1e7$}  & 1e-6    & \multicolumn{1}{l|}{1e7}   & 0.3, 1e-2           & \multicolumn{1}{l|}{1/300}     & 10         & \del{0.21/0.27ms}
\add{0.16/0/20ms}\\ 


\hline
\end{tabular}
}
\label{Table:statistics}
\end{table*}

%\subsubsection{Quatative Comparisons}
%We conduct a convergence rate comparison among methods for a single timestep, specifically midway through the sagging of a 15K vertex armadillo model. Our method is benchmarked against preconditioned gradient descent (GD) \cite{wang_descent_2016} and Newton's method. Additionally, we evaluate the convergence rate of the Jacobi version of our method, termed Block-Jacobi, implemented by computing $\Delta \vec{x}_k$ based on previous iteration positions for all the vertices simultaneously. For GD and Block-Jacobi, a line search is conducted every 8 iterations, while for Newton's method, a line search is performed in each iteration. For our method, GD and Block-Jacobi, both the Chebysev-accelerated and unaccelerated versions are examined. Notably, a fixed spectral radius $\rho=0.95$ is employed for acceleration. In our method, an iteration is defined as passing through all the colors.


%Compared to GD, our method demonstrates significantly faster convergence. Within a real-time frame of 33ms, our method achieves convergence to a relative error magnitude of 1e-4, whereas GD converges only up to a magnitude of 1e-2. Although Block-Jacobi shares similar computational costs with our method, it offers superior parallelism;\ziheng{Maybe we should be more specific about superior parallelism. Say all vertices can be computed at the same time.} however, in practice, it converges substantially slower than our method due to its Jacobi-iteration nature. Newton's method exhibits swift convergence in terms of iteration count but is notably the slowest in computational time, requiring 53ms per iteration, failing to meet real-time constraints.



\begin{comment}
    
\subsection{Stability with Large Residuals}

\begin{figure}
\centering
\newcommand{\img}[4]{\begin{subfigure}{0.33\linewidth}\centering
\fbox{\includegraphics[width=\linewidth,trim=#4,clip]{Figures/StabilityUnderResidual/#1-cc}}\vspace{-0.25em}
\caption{#2}\label{fig:StabilityUnderResidual:#3}
\end{subfigure}}
\newcommand{\figA}[3]{\img{#1}{#2}{#3}{450 100 550 300}}
\newcommand{\figB}[3]{\img{#1}{#2}{#3}{550 500 800 100}}
\figA{a}{GD, frame 5}{a}\hfill%
\figA{b}{\textbf{Ours}, frame 5}{b}\hfill%
\figA{c}{\textbf{Ours}, frame 100}{c}\vspace{0.5em}\\
\figB{d}{Newton, frame 5}{d}\hfill%
\figB{e}{\textbf{Ours}. frame 5}{e}\hfill%
\figB{f}{\textbf{Ours}, frame 100}{f} 
\caption{In this demonstration, we highlight stability in handling large residuals among various methods. These experiments involve a single iteration for a substantial time step of 1/60s. The top section exhibits an octopus undergoing gravitational sagging with its upper part fixed, showcasing outcomes from GD and our method. Meanwhile, the lower section illustrates the manipulation of a single vertex in an armadillo model, presenting results obtained using Newton's method and our method.}
\label{fig:StabilityUnderResidual}
\end{figure}


In our experiment depicted in \autoref{fig:StabilityUnderResidual}, we assess the stability of different methods in handling substantial residuals from prior frames using a large time step, permitting only one iteration per step. Specifically, in the upper section, we compare our method with GD as both handle an octopus undergoing gravitational sagging with fixed upper parts. GD fails by frame 5, while our method survives and continues running, albeit with noticeable overstretching artifacts by frame 100.
In the lower section, our method is contrasted with Newton's method, focusing on direct manipulation of a single vertex on an armadillo model's nose. Newton's method shows instability at frame 5, leading to explosive behavior, whereas our method adeptly manages abrupt manipulations. Note that here we switch to a LU factorization solver for Newton's method, combined with a PSD projection for the Hessains to best enhance the stability. Still, we found it very hard to make Newton's stable in this experiment. To make Newton's method, we have to take 10 smaller subteps and do multiple iterations per step.

In this experiment, both Newton's method and GD utilize a line search at each iteration, while our method adheres to a fixed step size of 1. 
It is important to note that while the line search ensures energy decrease within iterations during a single time step, it does not guarantee energy reduction between subteps.\ziheng{It is inappropriate to make statements about energy reduction between timesteps. Maybe change it to "does not guarantee stability in the long run".} As the optimization is reformulated at each time step, poor convergence from the previous frame can result in a subsequent step beginning with a substantial residual, potentially leading to explosive behavior even if the iteration successfully decreases the energy.

\end{comment}


\subsection{Comparisons to XPBD}

Our method has an entirely different formulation than XPBD, but there are some strong similarities, as both methods operate with position updates using Gauss-Seidel iterations. Here we provide two direct comparisons to highlight some important differences.


\begin{figure}
\centering
\newcommand{\img}[7]{\begin{subfigure}{0.245\linewidth}\centering
\includegraphics[width=\linewidth,trim=500 200 500 0,clip]{Figures/CompareToXPBD_TimeStep/#11-cc}\\
\includegraphics[width=\linewidth,trim=400 100 400 100,clip]{Figures/CompareToXPBD_TimeStep/#12-cc}
\caption{#3\\$h=1/#4$ sec.\\$n_{\max}=#5$\\$n_{\text{col}}=#6$\\\emph{($#7$ sec./frame)}}\label{fig:CompareToXPBD_TimeStep:#2}
\end{subfigure}}
\img{b}{a}{XPBD}{120}{120}{120}{0.32}\hfill%
\img{c}{b}{XPBD}{3000}{5}{125}{0.35}\hfill%1/3000 for collision detection
%\img{A00000059_}{c}{XPBD}{3000}{120}{1/125}{5.1}\hfill%
\img{d}{c}{XPBD}{3000}{5}{5}{3.1}\hfill%
\img{a}{d}{\textbf{VBD (ours)}}{120}{120}{120}{0.031}
\caption{A squishy ball with tentacles, comprising 230 thousand vertices and 700 thousand tetrahedra, dropped on the ground, simulated using \sref{a}~XPBD with a large time step and 240 iterations per frame, \sref{b}~XPBD with a $25\times$ smaller time step and 250 total iterations per frame, \sref{c}~XPBD with the same small time step and iteration count but with $25\times$ more frequent collision detection, and \sref{d}~VBD with a large time step and 240 iterations per frame. Comparing \sref{a} and \sref{d}, VBD is faster than XPBD with the same settings. XPBD's solution approaches VBD as the time step decreases, but it also requires more frequent collision detection to achieve a visually similar result to VBD.
%Comparative analysis with XPBD across various time steps. We explore the scenario involving the dropping of a squishy ball (comprising 230K vertices and 700K tetrahedra) onto the ground, generating numerous collisions. The blue tint highlights deeper penetrations caused by subsurface scattering artifacts due to intersecting geometry. The notations beneath each column denote: (the method name, collision detection time steps, elastic simulation time steps).
}
\label{fig:CompareToXPBD_TimeStep}
\end{figure}


XPBD replaces the Hessian matrix and uses only the Hessian of inertia potential. This omission is justified by using a small time step, because the significance of the inertia potential increases quadratically as the time step decreases. 
%
Nonetheless, with complex examples, the impact of this approximation can be severe, even with small time step.
%
This is demonstrated in \autoref{fig:CompareToXPBD_TimeStep} with a challenging collision-rich scenario involving a squishy ball with tentacles dropped to the ground. Comparing XPBD with 120 iterations per step (\autoref{fig:CompareToXPBD_TimeStep:a}) to our method with the same number of iterations (\autoref{fig:CompareToXPBD_TimeStep:d}), we can see that our method not only achieves a more stable animation, it also performs faster because of its improved parallelism, as compared to XPBD. Reducing the time step helps XPBD even when using a similar total number of iterations per frame (\autoref{fig:CompareToXPBD_TimeStep:b}). However, simply reducing the time step is not sufficient in this case, as XPBD also needs more frequent collision detection (\autoref{fig:CompareToXPBD_TimeStep:c}). Using collision detection with the same frequency as ours while taking small time step (\autoref{fig:CompareToXPBD_TimeStep:b}) leads to collisions that are detected too late and cause stability issues in this case. This is not only because the collisions that are detected too late are deeper, but also because smaller time step lead to higher vertex velocities when resolving stiff collisions.
%However, even when using 25$\times$ smaller time steps and 25$\times$ more iterations in total (\autoref{fig:CompareToXPBD_TimeStep:c}), it fails to match the result of our method. Nonetheless, we have observed that with more frequent collision detections, XPBD can eventually generate a result similar to ours in this example.

 

%Our method effectively simulates this scenario using a time step of 1/120s, conducting a single collision detection at the beginning of each step, resulting in a frame time of 0.11s (\autoref{fig:CompareToXPBD_TimeStep:a2}). In contrast, XPBD fails to handle such a sizable time step, compromising both the model's stiffness and collision handling abilities (\autoref{Fig:CompareToXPBD_TimeStep:b2}). Also, at this point, it is already slower than our method due to its high parallelization overhead. Simply decreasing the time step for elastic simulation while using the same collision detection time step does not work  (\autoref{fig:CompareToXPBD_TimeStep:c2}), as its collision handling demands increased collision detection frequency. To make the simulation work, XPBD necessitates a time step of 1/3000s for both elastic simulation and collision detection (\autoref{fig:CompareToXPBD_TimeStep:d2}), making it one magnitude slower than our method.



\begin{figure}
\centering
\newcommand{\figA}[3]{\begin{subfigure}{0.32\linewidth}\centering
\fbox{\includegraphics[width=\linewidth,trim=450 300 550 100,clip]{Figures/CompareToXPBD_MassRatio/#1}}
\caption{#2}\label{fig:CompareToXPBD_MassRatio:#3}
\end{subfigure}}
\figA{a}{Initial State}{a} \hfill%
\figA{b}{XPBD}{b} \hfill%
\figA{c}{\textbf{VBD (ours)}}{c} 
\caption{Dropping a large and heavy elastic cube onto a smaller and much lighter box with a mass ratio of 1:2000. Each cube has 400 vertices and 1.5 thousand tetrahedra.
%We compare our approach to XPBD concerning collision handling with a significant mass ratio scenario. This involves dropping a large box onto a smaller box, resulting in a collision between two sides with a mass ratio of 1:2000.\ziheng{change box to cube to match the article} 
}
\label{fig:CompareToXPBD_MassRatio}
\end{figure}


One of the fundamental challenges of XPBD is handling high mass ratios. This is demonstrated with a simple example in \autoref{fig:CompareToXPBD_MassRatio}, where a large and heavy elastic cube is dropped onto a smaller and much lighter cube, with a mass ratio of 1:2000. In this example, XPBD's collision constraints, even with infinite stiffness, cannot overcome the mass ratio and the smaller cube is entirely crushed upon contact. This is because of the dual formulation of XPBD \cite{macklin_primaldual_2020}. Our method, on the other hand, has no such difficulties with handling high mass ratios.

%In \autoref{fig:CompareToXPBD_MassRatio}, we contrast our method with XPBD regarding collision resolution in scenarios with a substantial mass ratio. Specifically, we observe the impact of dropping a large cube onto a significantly smaller cube, where the smaller cube's mass is merely 1/2000th of the larger one. In XPBD's simulation, the smaller cube is entirely crushed upon contact. In contrast, our method successfully represents the stiffness of the smaller cube, and successfully separates the two cubes. This disparity arises from XPBD's collision handling, which overlooks the material stiffness on both sides, relying solely on mass.




==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/05_Discussion.tex <==

%\section{Discussion}
\section{VBD for Other Simulation Systems}
\label{sec:othersims}
We have described our method in \autoref{sec:vbd} in the context of elastic body dynamics. Yet, VBD is not limited to such simulations and can be used to solve various optimization problems. Here, we consider some other example simulation systems and briefly discuss how our method can be applied. This is not intended as an exhaustive list but merely as examples that could guide the reader to discern how their specific simulation problem could utilize VBD.


\subsection{Particle-Based Simulations}
Particle-based simulations can easily use VBD by simply replacing the vertices in our description above with particles. Since VBD needs the Hessian of the force element energies, implementations would require computing the derivatives of all forces acting on a particle wrt. its position.

Parallelizing particle-based simulations also involves additional considerations.
%
Mass-spring type simulations, such as peridynamics \cite{Levine14}, can use our parallelization approach with vertex coloring.
%
However, simulations involving disjoint or loosely-joined particles, such as particle-based fluid simulation
%smoothed particle hydrodynamics 
\cite{Muller03,Takahashi15,Peer15}, would not only require recoloring at each time step but also using a conservative neighborhood definition (including \del{potential} position change within a time step) for coloring, since position updates can alter the set of \del{neighboring} particles that interact with each particle.
\begin{figure}
\centering
\newcommand{\img}[1]{\includegraphics[width=0.495\linewidth,trim=500 0 360 0, clip]{Figures/MassSpring/#1_combined-cc}}
\newcommand{\spc}{\hspace*{1em}}
\newcommand{\scap}[3]{\spc#1\hfill#2\spc\vspace{#3em}}
\img{Stiff}\hfill%
\img{Soft}\vspace{-3em}
\small\scap{stiff}{soft}{0}\\
\scap{springs}{springs}{1}\\
\caption{20 particles attached with springs, forming a swinging chain, simulated using VBD with a $S=1$ substep and $100$ iterations per step. The particle on one end of the chain is fixed and the particle on the other end has 1000$\times$ more mass than the others. \sref{Left}~using sufficiently stiff springs, they expand no more than 0.7\% of their rest lengths, despite the substantial mass difference. \sref{Right}~using 100$\times$ less stiff springs, the chain undergoes a visible expansion as it swings.}
\label{fig:massspring}
\end{figure}
\autoref{fig:massspring} shows a simple example where 20 particles, including one that is 1000$\times$ heavier, are connected with springs of two different stiffness, simulated using VBD.

\subsection{Rigid Body Simulation}

For handling rigid body simulations with VBD, we can replace each vertex in our formulation with an entire rigid body, using the variational formulation of rigid body dynamics \cite{Ferguson:2021:RigidIPC}. Unlike a vertex that has only 3 DoF, a rigid body also has rotational DoF, resulting in 6 DoF. Therefore, in our local system, we must solve a larger problem, where $\vec{x}_i \in  \mathbb{R}^{6}$ and $\Vec{H}_i \in \mathbb{R}^{6 \times 6}$, including Hessians of all force elements wrt. all 6 DoF of $\vec{x}_i$. Note that, in this case, these force elements are not internal material forces, but external forces acting on the rigid body, due to collisions or other constraints.
%Again, this 6D local system can be solved analytically or via the same numerical methods we discussed. \anka{analytical solver can be too expensive for a 6x6 system. We are not using this solver in our implementation. I suggest that we leave it as an open question.}

Other than this additional complexity, we can follow the same procedure with VBD. Parallelization with coloring depends on the nature of the rigid body simulation. For example, pre-coloring, as we used in our examples for elastic bodies might work for problems like a rigid body chain. For disjoint rigid bodies interacting through collisions only, dynamic recoloring might be needed.

Articulated rigid bodies can be handled by defining joint constraints with an elastic potential. 
Infinitely stiff constraints are also possible, but VBD cannot guarantee that they will be satisfied using a fixed number of iterations. Another alternative is 
hard constraints can be introduced by
reducing the total DoF in the system and replacing the vertices in our formulation with an articulated rigid body, having more than 6 DoF. Obviously, this would lead to an even larger local system, requiring modifications to the variational formulation. 
%and can be an interesting direction for future work.

\begin{figure}
\centering
\includegraphics[width=\linewidth,trim=100 200 100 120, clip]{Figures/RigidBody/chain-cc}
\caption{5 rigid bodies, each with 6 DoF, forming a chain through collisions, simulated using our VBD formulation for rigid body dynamics.}
\label{fig:rigidbody}
\end{figure}

\begin{figure}
\centering
%\includegraphics[width=\columnwidth]{Figures/08_ExtremeTwist.pdf}
% \includegraphics[width=\linewidth,trim=100 200 150 200, clip]{Figures/BeamRotation/a}\\
\newcommand{\img}[3]{\begin{subfigure}{0.498\linewidth}\centering
\includegraphics[width=\linewidth]
{Figures/TeapotOfRigid/#1}%\vspace{-0.5em}
\end{subfigure}}
\img{A0102}{180 0 150}{}\hfill%
\img{A0193}{180 0 150}{}
\img{A0272}{180 0 150}{}\hfill%
\img{A0720}{180 0 150}{}
\caption{Dropping 60 rigid bodies into a Utah teapot, showcasing collisions and frictional contact. Remarkably, one rigid body stays on the spout due to friction. }
\label{fig:RigidToTeapot}
\end{figure}

Example rigid body simulations are shown in \autoref{fig:rigidbody} and \autoref{fig:RigidToTeapot}, simulated using VBD, as described above.

Note that since our collision formulation is based on penetration potential, it corresponds to penalty forces. We leave the exploration of handling impulse-based collisions \cite{Mirtich96} with VBD to future work.



\begin{comment}
For this, we can use the variational formulation of rigid body dynamics \cite{Ferguson:2021:RigidIPC}, representing the variational energy of a single rigid body as
%
\begin{align}
    G_i(\vec{x}) &= E_{\vec{q}}(\vec{q}_i) + E_{\vec{Q}}(\vec{\bm\theta}_i) + E(\vec{x}) \;,
\end{align}
%
where $\vec{q}_i$ and $\vec{\bm\theta}_i$ are the translational and rotational DoF, respectively, such that ${\vec{x}_i=[\vec{q}_i\;\vec{\bm\theta}_i]^T}$, $E_{\vec{q}}$ and $E_{\vec{Q}}$ are the translation and rotational inertia potentials. Let $\vec{q}_i^t$ and $\vec{\bm\theta}_i^t$ be their values at the beginning of the time step, $\vec{Q}_i^t$ be the rotation matrix defined by $\vec{q}_i^t$, and $\vec{\dot{q}}_i^t$ and $\vec{\dot{Q}}_i^t$ represent linear and angular ve
%
\begin{align}
    \vec{\bar{q}}_i &= \vec{q}_i^t + h\vec{\dot{q}}
\end{align}
such that
%
\begin{align}
    E_{\vec{q}}(\vec{q}_i) &= \frac{m_i}{2h^2} \left\| \vec{q}_i - \vec{\bar{q}}_i \right\|^2 \\
    E_{\vec{Q}}(\vec{\bm\theta}_i) &=
    \frac{1}{2}\text{tr}(\vec{Q}_i\,\vec{J}_i\,\vec{Q}_i^T)
    - \text{tr}(\vec{Q}_i\,\vec{J}_i\,\vec{\bar{Q}}_i^T) \;,
\end{align}
%
where $\vec{\bar{q}}_i$
\end{comment}





%\subsection{Grid-Based or Mesh-Based Simulations}
%
%VBD can also be used for solving optimization problems defined on a grid or mesh, provided that the reduction in the optimized energy ($G$ in our formulation) can be represented using local energies ($G_i$ in our formulation). In this case, our vertices are replaced by grid cells or mesh nodes. Such problems can be easily parallelized, since the connections between cells and nodes typically remain constant.




\subsection{Unified Simulations}

Unified simulation systems are useful for handling scenarios that involve different material types. Typical unified simulation systems use a fundamental building block, such as a particle, to represent all supported materials \cite{Muller04,Solenthaler07,Becker09,Martin10,Macklin14}.
%
We can form a unified simulation system using VBD without representing all materials using the same building block.
%Unified simulation systems that combine simulations of different material types can be handled with VBD as well. 
For any simulation system described above, we can combine it with another, provided that we can define the information exchange as an energy potential.
For example, when the interactions take place as collisions, we can easily join rigid body simulations with elastic bodies or particles via the collision potential.
Joint constraints with elastic potential would be another easy way to combine different simulation systems. The advantage here is that a large rigid body, for example, can be represented as a single object with just 6 DoF, as opposed to using multiple building blocks that are constrained to move as a rigid construction.
%
This way, a heterogeneous collection of representations can be joined within the same integrator using VBD.

On the other hand, this form of defining a unified simulation system may be challenging for other types of information exchange, such as evaluating buoyancy. Exploring such problems would be another interesting direction for future research.



==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/06_Conclusion.tex <==

%\section{Limitations}
\section{Discussion}

\add{%
%\subsection{Block Coordinate Descent vs. Block Gauss-Sediel}
We derive our method as a block coordinate descent method for variational time integrators, which offers optimization techniques like PSD projection and line search. 
The fact that we do not require those techniques to guarantee stability actually makes our method a more general solver of nonlinear equations. 
When line search is not used, our method can effectively manage \textit{non-conservative forces}, such as friction, the same as how it handles conservative forces. 
In other words, our method allows for a seamless transition between block coordinate descent and block Gauss-Sediel \cite{hageman1975aspects, Grippo2000BlockGS}.  
While we do not practically utilize these optimization techniques derived from the descent view, they remain available options for users.}
%We encourage users to select these techniques based on the specific requirements of their use case scenario.


VBD is a descent-based method that operates through local iterations. Therefore, it may not be a good solution for problems that would benefit from a global treatment.

The speed of information travel with VBD depends on the connections of vertices and the number of iterations used. A perturbation applied on a vertex can impact other vertices of a connected chain through force elements at most as far as the number of colors within a single iteration. Therefore, VBD is not ideal for high-resolution stiff systems, as it may require too many iterations for a perturbation of a vertex to travel across the system. In such cases, a global solution using Newton's method may prove to be more effective.

%For relatively softer materials/connections, however, the speed of information travel is typically limited. That is why we are able to display superior convergence with VBD.

%Though VBD offers improved parallelization for Gauss-Seidel iterations through coloring vertices, as opposed to force elements/constraints, it still requires multiple parallel passes. Using Jacobi iterations with VBD would fix this, as our Block Jacobi version, but at the cost of significantly reduced convergence, as can be seen in \autoref{fig:ConvergenceComparisons}.

Our collision formulation for VBD is based on penetration potential. Therefore, it cannot guarantee penetration-free results. In fact, penetrations are almost never completely resolved, as some amount of penetration is needed to maintain some collision force. Exploring penetration-free collisions with VBD would be an interesting direction for future research.

In addition, defining a similar collision energy for codimensional objects, particularly for self-collisions, can be a challenge. 


\begin{figure}
\centering
\newcommand{\img}[5]{\begin{subfigure}{0.245\linewidth}
\includegraphics[width=\linewidth,trim=540 #4 540 #5, clip]{Figures/MassSpring/Rendered_#1_combined#2-cc}\vspace{-0.5em}
\caption{#3}
\end{subfigure}}
\newcommand{\imgA}[2]{\img{#1}{2}{#2}{380}{320}}
\newcommand{\imgB}[2]{\img{#1}{4}{#2}{100}{250}}
\imgA{100iters}{100 iterations}\hfill%
\imgA{converged}{Converged}\hfill%
\imgB{100iters}{100 iterations}\hfill%
\imgB{converged}{Converged}
\caption{A chain of particles connected with soft springs (orange) and 10,000$\times$ stiffer (blue) springs. Simulations with VBD using \sref{a,c}~100 iterations per frame fail to converge and result in excessive extensions, as compared to \sref{b,d}~converged results.}
\label{fig:stiffnessratios}
\end{figure}


VBD is a primal solver \cite{macklin_primaldual_2020}, so it can easily handle high mass ratios (see \autoref{fig:AdaptiveInitialization}, \ref{fig:CompareToXPBD_MassRatio}, and \ref{fig:massspring}), but it struggles with high stiffness ratios. This is shown in \autoref{fig:stiffnessratios} using a stiffness ratio of 1:10000, where VBD has poor convergence behavior.



\section{Conclusion}

We have presented vertex block descent, an efficient iterative descent-based solution for optimization problems, and described how it can be used for physics-based simulations with implicit Euler integration defined through a variational formulation.
%
We have explained all essential details of elastic body dynamics using VBD, including handling damping, constraints, collisions, and friction. We have defined an adaptive initialization technique, enabled by VBD's formulation, and discussed how to use momentum-based acceleration to improve convergence. We have also presented effective methods for parallelization using VBD, considering dynamically introduced/removed force elements, and explained how its vertex-level computation improves the parallelization of its Gauss-Seidel iterations.

Our results show that VBD can handle highly complex simulation cases (\autoref{fig:teaser}), it remains stable under extreme stress tests (\autoref{fig:ExtremeTwist}, \ref{fig:ExtremeInitialization}, \ref{fig:ExtremeStretch}, and \ref{fig:ExtremeStretch2}), and offers fast convergence (\autoref{fig:ConvergenceComparisons}). 

%We have also shown that VBD can handle high mass ratios (\autoref{fig:Initialization} and \ref{fig:CompareToXPBD_MassRatio}) \anka{Are we gonna put the mass spring pendulum in the paper or not}, a challenging condition for some prior methods \cem{shall we say "prior primal formulations?" We haven't quite declared our method as "primal" anywhere. Should we?}. \anka{I don't think this is a specific problem for primal formulation.}

In addition, we have summarized how VBD can be used for other types of simulation problems, such as particle systems and rigid bodies, including unified simulations. We have also mentioned some related future research directions and discussed VBD's limitations.



==> _Siggraph_2024__Vertex_Block_Descent_for_Elastic_Body_Dynamics/xx_ExampleFigures.tex <==
\clearpage
\begin{figure}
\centering
\newcommand{\figA}[3]{\begin{subfigure}{0.32\linewidth}\centering
\includegraphics[width=\linewidth,trim=450 100 550 300,clip]{Figures/StabilityUnderResidual/#1}
\caption{#2}\label{fig:StabilityUnderResidual:#3}
\end{subfigure}}
\newcommand{\figB}[3]{\begin{subfigure}{0.32\linewidth}\centering
\includegraphics[width=\linewidth,trim=600 200 700 100,clip]{Figures/StabilityUnderResidual/#1}
\caption{#2}\label{fig:StabilityUnderResidual:#3}
\end{subfigure}}
\figA{a}{GD at frame 5}{a} \hfill%
\figA{b}{ours at frame 5}{b} \hfill%
\figA{c}{ours at frame 100}{c} 
\figB{d}{Newton at frame 5}{d} \hfill%
\figB{e}{ours at frame 5}{e} \hfill%
\figB{f}{ours at frame 100}{f} 
\caption{In this demonstration, we highlight stability in handling large residuals among various methods. These experiments involve a single iteration for a substantial time step of 1/60s. The top section exhibits an octopus undergoing gravitational sagging with its upper part fixed, showcasing outcomes from GD and our method. Meanwhile, the lower section illustrates the manipulation of a single vertex in an armadillo model, presenting results obtained using Newton's method and our method.}
\label{fig:StabilityUnderResidual}
\end{figure}

==> xx_ExampleFigures.tex <==
\clearpage
\begin{figure}
\centering
\newcommand{\figA}[3]{\begin{subfigure}{0.32\linewidth}\centering
\includegraphics[width=\linewidth,trim=450 100 550 300,clip]{Figures/StabilityUnderResidual/#1}
\caption{#2}\label{fig:StabilityUnderResidual:#3}
\end{subfigure}}
\newcommand{\figB}[3]{\begin{subfigure}{0.32\linewidth}\centering
\includegraphics[width=\linewidth,trim=600 200 700 100,clip]{Figures/StabilityUnderResidual/#1}
\caption{#2}\label{fig:StabilityUnderResidual:#3}
\end{subfigure}}
\figA{a}{GD at frame 5}{a} \hfill%
\figA{b}{ours at frame 5}{b} \hfill%
\figA{c}{ours at frame 100}{c} 
\figB{d}{Newton at frame 5}{d} \hfill%
\figB{e}{ours at frame 5}{e} \hfill%
\figB{f}{ours at frame 100}{f} 
\caption{In this demonstration, we highlight stability in handling large residuals among various methods. These experiments involve a single iteration for a substantial time step of 1/60s. The top section exhibits an octopus undergoing gravitational sagging with its upper part fixed, showcasing outcomes from GD and our method. Meanwhile, the lower section illustrates the manipulation of a single vertex in an armadillo model, presenting results obtained using Newton's method and our method.}
\label{fig:StabilityUnderResidual}
\end{figure}
